A wireless signal-based sensing framework for robotics

In this paper we develop the analytical framework for a novel Wireless signal-based Sensing capability for Robotics (WSR) by leveraging robots' mobility. It allows robots to primarily measure relative direction, or Angle-of-Arrival (AOA), to other robots, while operating in non-line-of-sight unmapped environments and without requiring external infrastructure. We do so by capturing all of the paths that a wireless signal traverses as it travels from a transmitting to a receiving robot in the team, which we term as an AOA profile. The key intuition behind our approach is to enable a robot to emulate antenna arrays as it moves freely in 2D and 3D space. The small differences in the phase of the wireless signals are thus processed with knowledge of robots' local displacement to obtain the profile, via a method akin to Synthetic Aperture Radar (SAR). The main contribution of this work is the development of i) a framework to accommodate arbitrary 2D and 3D motion, as well as continuous mobility of both signal transmitting and receiving robots, while computing AOA profiles between them and ii) a Cramer-Rao Bound analysis, based on antenna array theory, that provides a lower bound on the variance in AOA estimation as a function of the geometry of robot motion. We show that allowing robots to use their full mobility in 3D space while performing SAR, results in more accurate AOA profiles and thus better AOA estimation. All analytical developments are substantiated by extensive simulation and hardware experiments on air/ground robot platforms using 5 GHz WiFi. Our experimental results bolster our analytical findings, demonstrating that 3D motion provides enhanced and consistent accuracy, with total AOA error of less than 10 degree for 95% of trials. We also analytically characterize the impact of displacement estimation errors on the measured AOA.

==> text/CRB_v2.tex <==
\section{Analysis of Trajectory Impact on Relative AOA Measurements}\label{sec:Analysis_impact_factors}
We establish theoretical performance bounds of our system as they relate to the AOA profile, $F_{ij}(\phi,\theta)$, accuracy. We do so by characterizing the effect of robot trajectories on the resulting accuracy of obtained $AOA_{max}$ measurements that correspond to strongest signal direction, which is the direct signal path in our case. Two major factors that we analyze are the impact of \emph{trajectory geometry} and the impact of \emph{trajectory estimation errors} on the resulting $AOA_{max}$ accuracy. Along these lines, in this section we independently analyzing the following factors:
\begin{enumerate}
    \item \textbf{\emph{Trajectory geometry (2D, 3D)}}: To analyze the system performance due to variations in trajectory geometry in ideal conditions, we formulate the Cramer-Rao bound for a \emph{3D helix} as well as the two special cases of \emph{Planar Curve} and \emph{Linear} trajectories in Sec.~\ref{sec:cr-bound}. Our analysis shows that 3D trajectories lead to generally lower variance (higher \emph{informativeness}) in $F_{ij}(\phi,\theta)$ compared to 2D trajectories.
    \item \textbf{\emph{Trajectory estimation errors}}: We analyze the performance of our system in the presence of both constant and varying position estimation error in the trajectory.  We derive the mathematical relation between position estimation error and error in the $F_ij(\phi,\theta)$ in Sec.~\ref{sec:characterization-trajectory-err-analysis}. 
    % \item \textbf{\emph{Trajectory discretization}}: Trajectory estimates that have variation of spacing between positions and the bursty nature of WiFi packets results in discretization of the virtual antenna array elements, thus impacting AOA estimation due to manifestation of anomalous peaks in the AOA profile. In Sec.~\ref{sec:Trajectory_discretization}, we analyze the extent to which discretization can be tolerable so that the main peak corresponding to the strongest signal direction remains identifiable.
\end{enumerate}
\noindent Although for the purposes of analysis we analyze these factors separately, in reality all of these factors will act simultaneously to impact the accuracy of the resulting $F_{ij}(\phi,\theta)$. Our extensive empirical analyses from hardware experiments include simultaneous impact of both factors however, and demonstrates agreement with all analytical results presented in this paper.

\subsection{Cramer Rao Bound for different trajectory geometries}\label{sec:cr-bound}
Here, we consider the impact of the robots' trajectory shape on \emph{AOA} estimation. Our main tool of analysis here will be the Cramer Rao Bound (CRB) which provides a lower bound on the variance of the $AOA_{max}$ estimation for a given trajectory shape as captured by the steering vector $\textbf{a}(\phi,\theta)\textbf{(t)}$ (cf. Eqn.~\eqref{eqn:steering_vector}). This variance is inversely proportional to the \emph{Informativeness} of the trajectory such that a lower variance indicates higher informativeness for a given trajectory shape (cf. Defn.~\ref{def:Informativeness}). We note that the CRB is a function of source location at a given $(\phi,\theta)$. In other words, the variance of the resulting $AOA_{max}$ estimate is a function of the different relative directions between the transmitting and receiving robots. Intuitively, depending on the shape of the antenna array (dictated in our case by the receiving robot's trajectory), the phase differences in the received signal will be easier or harder to discern. In this section we analyze this discerning capability of different trajectories via the CRB.  Specifically, in this section we develop a closed-form formulation of the CRB as a function of both trajectory as given by $\textbf{a}(\phi,\theta)\textbf{(t)}$, and relative direction of the transmitting robot i.e $(\phi,\theta)$.

We start by deriving the general form of the CRB for arbitrary robot trajectories. Given that $\mathbf{h_{ij}(t)}$ is complex, deterministic, and known at the receiver robot, it is clear from Eqn. \ref{eq:array_model} that  output model \textbf{Y(t)} satisfies the \emph{Conditional observation model}; i.e. it is multivariate Gaussian with mean $\textbf{a}(\theta,\phi)\textbf{(t)}~\mathbf{h_{ij}(t)}$ and variance $\sigma^2I$~\citep{Vu2013-3D}. Thus, the expression for the CRB for an arbitrary 3D geometry array can be found in~\citep{Vu2010PerformanceAO} as given in Eqn. \ref{eq:CRB_equation} (dropping the notation $t$ and subscript $i,j$ for brevity):
\begin{align*}
&\hspace{-3.2in}\text{CRB} = \frac{\sigma^2}{2\mathbf{h}^H\mathbf{h}} \times \\
% \begin{bmatrix}
% C_{\theta \theta} & C_{\theta \phi} \\
% C_{\phi \theta} & C_{\phi \phi} \\
% \end{bmatrix}\\
{\underbrace{
\begin{bmatrix}
\underbrace{Re(\frac{\partial \textbf{a}^H(\theta,\phi)}{\partial\theta} \frac{\partial \textbf{a}(\theta,\phi)}{\partial\theta})}_{\textbf{A}}  & 
\underbrace{Re(\frac{\partial \textbf{a}^H(\theta,\phi)}{\partial\theta} \frac{\partial \textbf{a}(\theta,\phi)}{\partial\phi})}_{\textbf{C}} \\
\underbrace{Re(\frac{\partial \textbf{a}^H(\theta,\phi)}{\partial\phi} \frac{\partial \textbf{a}(\theta,\phi)}{\partial\theta})}_{\textbf{C}} & \underbrace{Re(\frac{\partial \textbf{a}^H(\theta,\phi)}{\partial\phi} \frac{\partial \textbf{a}(\theta,\phi)}{\partial\phi})}_{\textbf{B}}
\end{bmatrix}
}_{FIM}}^{-1}
\end{align*}
where $\mathbf{h}^H\mathbf{h}$ = $\norm{h}^2$ is signal magnitude, and $Re$ stands for real number. It is also inversely proportional to the FIM (Fisher Information Matrix), as indicated above. Following the development in~\citep[Sec. 6]{Vu2010PerformanceAO}, derivatives of the $u^{th}$ element of the steering vector with $M$ total elements are given as:
\begin{align*}
    &\frac{\partial a_u(\theta,\phi)}{\partial \theta}= \\ 
    &\frac{2\pi \rho_u \Upsilon_u\sqrt{-1}}{\lambda}(\cos\theta \sin\xi_u\cos(\phi-\varphi_u)-\cos\xi_u\sin\theta)
\end{align*}
\begin{align*}
    \frac{\partial a_u(\theta,\phi)}{\partial \phi}=-\frac{2\pi \rho_u \Upsilon_u\sqrt{-1}}{\lambda}(\sin\theta \sin\xi_u\sin(\phi-\varphi_u)
\end{align*}
\noindent where 
\begin{align*}
    \Upsilon_u=e^{\frac{2\pi \rho_u\sqrt{-1}}{\lambda}(\sin\theta\sin\xi_u\cos(\phi-\varphi_u)+\cos\xi_u\cos\theta)}
\end{align*}

\smallskip
\noindent After some simplification the partial derivative terms in the FIM become:
\begin{align*}
&\hspace{-3.0in}\textbf{A} = \frac{\partial \textbf{a}^H(\theta,\phi)\partial \textbf{a}(\theta,\phi)}{\partial\theta \partial\theta}=\\
\sum_{u=1}^M \frac{4\pi^2 \rho_u ^2}{\lambda^2}(\cos\theta \sin\xi_u \cos(\phi - \varphi_u)-\cos\xi_u\sin\theta)^2
\end{align*}
and:
\begin{align*}
&\hspace{-2.5in}\textbf{B} = \frac{\partial \textbf{a}^H(\theta,\phi)\partial \textbf{a}(\theta,\phi)}{\partial\phi \partial\phi}= \\
\hspace{-.2in}\sum_{u=1}^M \frac{4\pi^2 \rho_u ^2}{\lambda^2}(\sin\theta \sin\xi_u \sin(\phi - \varphi_u))^2
\end{align*}
and finally:
\begin{align*}
&\hspace{-3.1in} \textbf{C} = \frac{\partial \textbf{a}^H(\theta,\phi)\partial \textbf{a}(\theta,\phi)}{\partial\phi \partial\theta}=\\
\hspace{.2in}\sum_{u=1}^M \frac{4\pi^2 \rho_u ^2}{\lambda^2}(\cos\theta \sin\xi_u \cos(\phi - \varphi_u)-\cos\xi_u\sin\theta)\\
\times (\sin\theta \sin\xi_u \sin(\phi - \varphi_u))
\end{align*}

\noindent Taking the determinant of the FIM, we arrive at the general form for the CRB in each the $\theta$ and $\phi$ directions:
\begin{align}
CRB_\theta = \frac{\sigma^2}{2\norm{h}^2Det(FIM)\textbf{A}} \nonumber \\
CRB_\phi =\frac{\sigma^2}{2\norm{h}^2Det(FIM)\textbf{B}}
\label{eq:CRB_helix_closed_form}
\end{align}
where $\sigma^2$ is the variance of our noise and \norm{h} is the magnitude of our signal, that is, $\frac{\sigma^2}{2\norm{h}^2}$ = $\frac{1}{\text{SNR}}$, where SNR is the signal to noise ratio.
% \begin{align*}
%     \frac{\sigma^2}{\norm{h}} = \frac{1}{\text{SNR}}
% \end{align*}

\medskip
\noindent In the following sections, we include specific forms of the CRBs for three types of symmetrical trajectory geometries that can be obtained on robot platforms - 2D linear, 2D curved and a 3D helix, to obtain in-depth insights on how their corresponding CRB values impact relative AOA. In section \ref{sec:results_informativeness} we show that these insights generalize well for arbitrary shaped 2D and 3D trajectories. Detailed derivations of CRB for these trajectories can be found in Appendix section \ref{sec:CRB_math}.
%====CRB analysis figure====
\begin{figure*}
	\centering
	\begin{minipage}{.4\linewidth}
		\includegraphics[height=4cm]{Images/CRBPhi.png}
        %\vspace*{-0.2in}
        \footnotesize\emph{{(a) Cramer-Rao Bound for a simulated receiving robot trajectory in $\phi$ (azimuth) direction}}
	\end{minipage}
	    \hspace{10pt}
		\begin{minipage}{.4\linewidth}
		\includegraphics[height=4cm]{Images/CRBTheta.png}
		\footnotesize\emph{{(b) Cramer-Rao Bound for a simulated receiving robot trajectory in $\theta$ (elevation) direction}}
        %\vspace*{-0.2in}
    \end{minipage}
% 	\hfill%
% 	\begin{minipage}{.32\linewidth}
% 		\centering
%		\includegraphics[height=4.3cm]{SigmaTheta.pdf}
 %       \vspace*{-0.3in}
%		\caption{Effect of Angular Displacement on Cramer-Rao Bound Stdev of Error for a path of fixed length, across various $\theta$ with a fixed target SNR and $\phi$}
%		\label{fig:cr-theta}
% 	\end{minipage}
	\caption{\footnotesize{\emph{CDF plot showing the effect of trajectory shape on Cramer-Rao Bound in the (a) $\phi$ direction and (b) $\theta$ direction for a receiving robot's simulated trajectory of fixed length, from 129600 simulated locations of transmitting robot that are uniformly distributed in 3D space. We see that 3D trajectory (helix) has a tighter bound compared to 2D trajectories (circle and line). Cumulative result from hardware experiments (Fig.~\ref{fig:CRB_vs_AOA_error}) demonstrates that indeed the \emph{informativeness} calculated for each trajectory (inverse of the CRB) successfully captures the improved performance in AOA estimation for 3D versus 2D trajectories.}}}
	\label{fig:cr-theta-phi}
\end{figure*}
%====CRB analysis figure====

\subsubsection{\textbf{Analysis of special geometries.}}
\paragraph{(a) [3D spherical helix].} We begin by considering the case of a 3D spherical helix trajectory to build intuition on the impact of 3D trajectories on the CRB. For such a trajectory, its spherical coordinates are given by (dropping $t$ and subscript $i$ for brevity):
\begin{align*}
   \xi_u= \tau, \hspace{0.1in} \varphi_u= c\tau, \hspace{0.1in}
   \rho_u= r
    \end{align*}
for a spherical helix of radius $r$, spiral climb rate of $c$, and parameterization $\tau\in[0,2\pi)$. We assume that each antenna element $u$ is uniformly spaced along the helix so that $\tau=\{0,\Delta,2\Delta,\hdots,(M-1)\Delta\}$ where $\Delta=\frac{2\pi}{M}$. Further, we assume a climb rate  $c=1$ for a simplification of our closed form, though any constant can be similarly substituted before integration. So for our 3D spherical helical trajectory, our CRB terms become:
\begin{align*}
    &\hspace{-0.1in}\textbf{A}=-\frac{\pi ^2 r^2 \left(\cos ^2(\theta ) \cos (2 \phi )+\cos (2 \theta )-3\right)}{\lambda ^2}
\end{align*}
\begin{align*}
    &\hspace{-0.9in}\textbf{B} = \frac{\pi ^3 r^2 \sin ^2(\theta ) (\cos (2 \phi )+2)}{\lambda ^2}
\end{align*}
\begin{align*}
    &\hspace{-0.4in}\textbf{C}=\frac{2 \pi ^3 r^2 \sin (\theta ) \cos (\theta ) \sin (\phi ) \cos (\phi )}{\lambda ^2}.
\end{align*}

\noindent The Fisher Information for $\theta$ and $\phi$ are given by $\frac{2\norm{h}^2}{\sigma^2}$\textbf{A} and $\frac{2\norm{h}^2}{\sigma^2}$\textbf{B} respectively~\citep{Vu2013-3D}.
We calculate the determinant of FIM as follows:
\begin{align*}
&\textbf{Det}(\text{FIM}) = \\ &\frac{\pi ^5 r^4}{8 \lambda ^4} \sin ^2(\theta ) (8 \cos (2 (\theta -\phi ))+8 \cos (2 (\theta +\phi ))\\
& +\pi  \cos (2 (\theta +2 \phi ))+\cos (2 (\theta +2 \phi ))\\
&+(1+\pi ) \cos (2 (\theta -2 \phi ))\\
& -2 (\pi -9) \cos (2 \theta )-16 \cos (2 \phi )+2 \pi  \cos (4 \phi )\\
&+2 \cos (4 \phi )-2 \pi +50)
\end{align*}

\noindent Substituting \textbf{A}, \textbf{B}, and \textbf{Det}(FIM) into Eqn. \ref{eq:CRB_helix_closed_form} thus gives the corresponding closed form equation of the CRB for a spherical helix (Derivation in Appendix \ref{sec:CRB_math} (I)).

\paragraph{(b) $z=0$ [Planar circular trajectory].} For $z=0$ the helix is a circle of radius $r$ and the CRB equations should be the same as a circular planar curve.  For this case we have (dropping $t$ and subscript $i$ for brevity): 
\begin{align*}
    \xi_u= \tau,\hspace{0.1in} \rho_u=r,\hspace{0.1in} \varphi_u=\cos^{-1}(0)=\pi/2
\end{align*}

The CRB equations reduce to
\begin{align*}
    \textbf{A}= \frac{2\pi^2r^2}{\lambda^2}\cos^2\theta
\end{align*}
\begin{align*}
    \textbf{B}=\frac{2\pi^2r^2}{\lambda^2}\sin^2\theta
\end{align*}
\begin{align*}
    \hspace{-0.5in}\textbf{C}=0.
\end{align*}
% %====CDF plots====
% \begin{figure*}
% 	\centering
% 	\begin{minipage}{.47\linewidth}
%         \includegraphics[width=8.0cm,height=6.0cm]{Images/CDF_phi2.png}
% 	\end{minipage}
% 	\hspace{15pt}
% 	\begin{minipage}{.47\linewidth}
% 		\centering
%         \includegraphics[width=8.0cm,height=6.0cm]{Images/CDF_theta2.png}
% 	\end{minipage}
% 	\caption{\footnotesize{\emph{CDF plot for Angle-of-Arrival estimation error in azimuth $\phi$ (left) and elevation $\theta$ (right) angles for 2D and 3D (green) trajectories obtained from a total of 303 hardware experiments. 2D curved trajectories and 3D trajectories have similar accuracy in azimuth but differ for elevation accuracy (see Fig.~\ref{fig:Traj_informativeness} for wireless signal profile ambiguities). 2D linear trajectories perform the worst in both azimuth and elevation.}}}
%     \label{fig:CDF_phi_theta}
% \end{figure*}
% %====CDF plots====

\noindent Substituting the values \textbf{A} and \textbf{B} in Eqn. \ref{eq:CRB_helix_closed_form} gives the corresponding closed form equation of the CRB for the planar circular trajectory (Derivation in Appendix \ref{sec:CRB_math} (II)).

\medskip
\paragraph{(c) $r\rightarrow\infty$ [Planar linear trajectory].} For simplicity, we consider a line segment of length $2\pi$r at angle (a, b). This is parameterized in spherical coordinates as follows (dropping $t$ and subscript $i$ for brevity):
\begin{align*}
   \xi_u = a,\hspace{0.1in} \varphi_u= b,\hspace{0.1in} \rho_u= r\tau
\end{align*}
% %====MOcap_vs_Camera_AOA_accuracy====
% \begin{figure*}
% 	\centering
% 	\begin{minipage}{.45\linewidth}
%         \includegraphics[width=8.0cm,height=5.0cm]{Images/Effect_of_trajectory_estimation_error_on_AOA_error.png}
%     	\caption{\footnotesize{\emph{AOA for actual trajectory using motion capture(blue) versus estimated trajectory using camera (orange).}}\textcolor{red}{\textbf{Sec: Characterization of trajectory error. Reference text in Results sub-section D}}}
%     	%$\Phi$=\ang(-90), $\Theta$=\ang(90), denoted by red 'x'}
%     	\label{fig:Traj_comparison}
% 	\end{minipage}
% 	\hspace{20pt}
% 	\begin{minipage}{.45\linewidth}
% 		\centering
%          \includegraphics[width=8.0cm,height=5.5cm]{Images/Mocap_vs_camera_AOA.png}
%     	 \caption{\footnotesize{\emph{Aggregate results of AOA estimation for 59 experiments. Groundtruth azimuth angle $\phi$ = \ang{0} and elevation angle $\theta$ = \ang{91}}}\textcolor{red}{\textbf{Sec: Results}}}
%         	\label{fig:Mocap_vs_camera_AOA}
% 	\end{minipage}
% \end{figure*}

Thus, our CRB terms are:
\begin{align*}
&\hspace{-0.27in}\textbf{A}=\sum_{u=1}^M \frac{4\pi^2 (r(u-1)\Delta) ^2}{\lambda^2}\\
&(\cos\theta \sin(r(u-1)\Delta)\cos(\phi - b)-\cos(a)\sin\theta)^2
\end{align*}

\begin{align*}
&\hspace{-0.4in}\textbf{B}= \sum_{u=1}^M \frac{4\pi^2 (r(u-1)\Delta) ^2}{\lambda^2}(\sin\theta \sin(a) \sin(\phi - b))^2
\end{align*}

\begin{align*}
&\hspace{-0.47in}\textbf{C}=\sum_{u=1}^M \frac{4\pi^2 (r(u-1)\Delta) ^2}{\lambda^2} \\ &*(\cos\theta \sin(a) \cos(\phi - b)-\cos(a)\sin\theta)\\
&\hspace{-0.1in}* (\sin\theta \sin(a) \sin(\phi - b))
\end{align*}

\noindent We do not show a closed form for the CRB for a line, as the `u' term is not inside a trigonometric function and the CRB quickly inflates to infinity, except in certain directions where the trigonometric terms go to zero. That is, depending on the direction, linear trajectories are largely uninformative.
%====MOcap_vs_Camera_AOA_accuracy====
\begin{figure*}
	\centering
    \includegraphics[width=16.3cm,height=8.5cm]{Images/Effect_of_trajectory_estimation_error_on_AOA_error.png}
	\caption{\footnotesize{\emph{ Shows the AOA profile $F_{ij}(\phi,\theta)$ using groundtruth and Intel Realsense T265 tracking camera trajectories obtained from hardware experiment. The peak $AOA_{max}$ in the in $F_{ij}(\phi,\theta)$ corresponds to the strongest signal direction of transmitting robot. Error in the estimated trajectory increases the error in $AOA_{max}$ estimation and results in a more noisy profile (top right). The groundtruth AOA angles are marked by red 'x' in the Top View of the $F_{ij}(\phi,\theta)$. We see that there is a clear attenuation of the $AOA_{max}$ and a slight shift for the tracking camera trajectory compared to the peak obtained from groundtruth trajectory. Aggregate results comparing the groundtruth and tracking camera trajectories are shown in Fig. \ref{fig:Mocap_vs_camera_AOA}.}}}  
	%$\Phi$=\ang(-90), $\Theta$=\ang(90), denoted by red 'x'}
	\label{fig:Traj_comparison}
\end{figure*}
%====MOcap_vs_Camera_AOA_accuracy====

\subsubsection{\textbf{Observations:}}
We note a few observations from our analysis by comparing the 2D circle to the 3D helix. The off-diagonal terms of our CRB matrix (Eqn. \ref{eq:CRB_equation}), are always zero for the case of 2D circle. This results in a decoupling of the CRB in the $\theta$ and $\phi$ directions. When the transmitting robot is located in the x-y plane i.e $\theta=\frac{\pi}{2}$, $CRB_{\theta}$ for the planar circular case tends to infinity (as the \textbf{A} term becomes 0) while it remains finite for the 3D geometry case, thus the variance for the 2D trajectory increases (i.e. its informativeness decreases) as compared with the 3D trajectory case for some relative angles between receiving and transmitting robots. The high variance in performance of AOA estimation for the planar 2D case is sometimes referred to as the ambiguity problem of planar circular trajectory along elevation direction \citep{Vu2013-3D}. Note that this is not the case for 3D trajectories which do not experience a variance increasing arbitrarily high for any transmitting robot locations relative to receiving robot. This theoretical finding is supported by hardware experiments (Fig. \ref{fig:Traj_ambiguity}) which shows that 2D curved trajectories are more ambiguous along $\theta$. Further, we note the \textbf{B} term for a helix is always higher than for the planar circle by a factor of at least $\pi$, which results in a tighter bound for $\phi$ for a helical trajectory.

In addition to observations from our derivation, we also note some observations on the CRB from simulated trajectories of receiving robot. This data was collected by simulating trajectories of a fixed length in each of the aforementioned shapes: a circle, a line, and a spherical helix. Then, the Cramer-Rao Bound (cf. Eqn. \ref{eq:CRB_helix_closed_form}) was calculated for a simulated transmitting robot in each angular position between 1 and 360 degrees in each the $\phi$ and $\theta$ directions, for a total of 129600 possible transmitting robot locations. The CDF of the CRBs across all positions are shown in Fig.~(\ref{fig:cr-theta-phi}). We see the tightest bound on the helix, followed by the circle and then the line, thus ranking these common trajectories in terms of informativeness.
% This theoretical finding is supported by hardware experiments (Fig. \ref{fig:Traj_ambiguity}) which shows that 2D curved trajectories are more ambiguous along $\theta$ and leading to high AOA error in elevation (Fig. \ref{fig:CDF_phi_theta} (c)). Cumulative results from hardware experiments (Fig. \ref{fig:CDF_phi_theta} (b)) also indicate that 3D trajectories have comparatively higher accuracy than 2D trajectories along the azimuthal angle ($\phi$).

%\textcolor{red}{[SG Question: is this next paragraph still relevant or not anymore since we have updated these figures?]} In Fig.~\ref{fig:cr-snr} and Fig. \ref{fig:cr-phi}, we show our results for the Cramer-Rao bound across different 2-D simulated trajectories. For these, we show CRBs of paths of arcs of fixed length with varying angular displacements in elevation and azimuth from 0.01$\pi$ (approximating a straight line) to 2$\pi$ (a circle), across a few different target positions. This supports our observation of lines in certain directions approaching infinitely unbounded by the CRB, as is shown in the $\phi=\frac{\pi}{2}$ case. Further, this shows an improvement of the CRB for arcs rather than full circles for a path of given length.

%We make the following observations:
%\begin{enumerate}
%    \item $\phi$ appears to have the effect of magnifying the error, while the overall trajectory geometry is preserved. 
%    \item Local maximum in error position determined by $\theta$, suggesting the \textit{least} optimal curvature of a path varies $\theta$, which makes sense as the trajectory of curved line appears most straight at a given $\theta$.
%\end{enumerate}
%We note that these errors converge when \textcolor{red}{the angular displacement is 2$\pi$,since differences in path are eliminated when the device rotates in a full circle \textbf{NEED REVIEW}}. However, this unified Cramer-Rao bound is not the most optimal path for a given $\theta$, suggesting that advancements can be made in algorithms to improve the shape of a SAR trajectory.

% Results from hardware experiments agree with the conclusions drawn from our theoretical analysis. Cumulative results that relate $AOA_{Error}$ with CRB (Fig.~\ref{fig:CRB_vs_AOA_error}) show that 3D trajectories have comparatively higher \emph{informativeness} as they have lower CRB and $AOA_{Error}$. An empirical CDF plot generated from a total of 101 trajectory samples each for three different types of hardware trajectories (Fig. \ref{fig:CDF_phi_theta} (a)) clearly shows that arbitrary 3D trajectories have less than $\ang{10}$ $AOA_{Error}$ for 95\% of the total trajectory samples of that type, where as only 50\% of 2D curved trajectories and 7\% of 2D linear trajectories show similar accuracy. Additionally, comparing ambiguity in AOA profile for three sample trajectories of each type (Fig.~\ref{fig:Traj_ambiguity}), we see that a 2D linear trajectory results in ambiguity in both $\phi$ and $\theta$. On the other hand, 2D curved trajectories results in ambiguous $\theta$ and a 3D trajectory eliminates all ambiguities.


==> text/abstract.tex <==
\begin{abstract}
In this paper we derive a new capability for robots to measure relative direction, or Angle-of-Arrival (AOA), to other robots, while operating in non-line-of-sight and unmapped environments, without requiring external infrastructure. We do so by capturing all of the paths that a WiFi signal traverses as it travels from a transmitting to a receiving robot in the team, which we term as an \emph{AOA profile}. The key intuition behind our approach is to \emph{emulate antenna arrays in the air} as a robot moves freely in 2D or 3D space. The small differences in the phase and amplitude of WiFi signals are thus processed with knowledge of a robots' local displacements (often provided via inertial sensors) to obtain the profile, via a method akin to Synthetic Aperture Radar (SAR). The main contribution of this work is the development of i) a framework to accommodate arbitrary 2D and 3D trajectories, as well as continuous mobility of both transmitting and receiving robots, while computing AOA profiles between them and ii) an accompanying analysis that provides a lower bound on variance of AOA estimation as a function of robot trajectory geometry that is based on the Cramer Rao Bound and antenna array theory. This is a critical distinction with previous work on SAR that restricts robot mobility to prescribed motion patterns, does not generalize to the full 3D space, and/or requires transmitting robots to be static during data acquisition periods. In fact, we find that allowing robots to use their full mobility in 3D space while performing SAR, results in \emph{more accurate} AOA profiles and thus better AOA estimation. We formally characterize this observation as the \emph{informativeness of the trajectory}; a computable quantity for which we derive a closed form. All theoretical developments are substantiated by extensive simulation and hardware experiments on air/ground robot platforms. Our experimental results bolster our theoretical findings, demonstrating that 3D trajectories provide enhanced and consistent accuracy, with AOA error of less than $10\deg$ for $95\%$ of trials. We also show that our formulation can be used with an off-the-shelf trajectory estimation sensor (Intel RealSense T265 tracking camera), for estimating the robots' local displacements, and we provide theoretical as well as empirical results that show the impact of typical trajectory estimation errors on the measured AOA. Finally, we demonstrate the performance of our system on a multi-robot task where a heterogeneous air/ground pair of robots continuously measure AOA profiles over a WiFi link to achieve dynamic rendezvous in an unmapped, 300 square meter environment with occlusions.
\end{abstract}




==> text/approach.tex <==
%=========Forward-Reverse Representation===
\begin{figure}
  \centering
  \includegraphics[width=7.0cm,height=5.0cm]{Images/forward_backward.PNG}
  \caption{\footnotesize{\emph{Schematic representation of forward channel (from robot $i$ to robot $j$) and reverse channel (from robot $j$ to robot $i$). This enables our system to cancel the Carrier Frequency Offset (CFO).}}}
  \label{fig:foward_reverse}
\end{figure}
%=========Forward-Reverse Representation===
\section{SAR for Arbitrary Trajectories}\label{sec:Development}
Trajectory estimation methods generally result in substantial orientation and position errors $R_{\epsilon}(t)$ and $p_{\epsilon}(t)$ for longer trajectories and without loop closures~\citep{drift_slam}. We use local sub-trajectory estimate $\boldmath{\hat{\chi_i}}\textbf{(t)}$ for receiving robot $i$ over $M$ robot positions $p_i(t_k),\hdots,p_i(t_l)$, $l=k+M$, in order to obtain the AOA profile $F_{ij}(\phi,\theta)$ (e.g. Fig.~\ref{fig:3D_SAR_AOA}) for \emph{arbitrary motion} in 2D and 3D. In practice $M$ can be about 200 packets collected over a few seconds and the length of the local sub-trajectory should be $\geq$ 2$\lambda$. We define the residual error $\epsilon(t)$ for any pose in $\boldmath{\hat{\chi_{i}}}\textbf{(t)}$ as follows: 
\begin{definition}[\underline{Residual Error}]: Given error $p_{\epsilon}(t_k)$ in position $p(t_k)$ for the first pose $\hat{\chi_i(t_k)}$ in $\boldmath{\hat{\chi_i}}\textbf{(t)}$, for any time $t\in[t_k,\hdots,t_l]$, the residual error is given as $\epsilon(t)$ = $p_{\epsilon}(t)$ - $p_{\epsilon}(t_k)$.
\label{def:residual_error}
\end{definition}
\noindent As stated in our assumptions all measurements are with respect to $p_i(t_k)$. Thus, a position $p_i(t_u)$ at timestep $t_u$ in the sub-trajectory becomes: 
\begin{align*}
p(t_{uk}) + \epsilon(t_{u}) = p(t_{u}) - p(t_{k}) + p_\epsilon(t_{u}) - p_\epsilon(t_{k}) 
\end{align*}
where $p_i(t_{uk})$ is position $p_i(t_{u})$ relative to the position at time $p_i(t_{k})$ and $\epsilon(t_{u})$ is the residual error. Note that our system is not impacted by orientation errors since it uses an omnidirectional antenna. In other words, our system is only impacted by the accumulation of residual errors (and trajectory geometry as discussed in Sec. \ref{sec:Analysis_impact_factors}). For the rest of the paper any position $p_i(t_{u})$ for a robot $i$ is implicitly assumed to be $p_i(t_{uk})$ for brevity. 

Given a perfect trajectory estimation $\boldmath{\chi_i}\textbf{(t)}$, the errors terms can be set to zero as in the case of using a motion capture system. We redefine the steering vector $\textbf{a}(\theta,\phi)\textbf{(t)}$ from Eqn. \ref{eqn:steering_vector_eqn_basic} in spherical coordinates as follows: (dropping the notation $t$ and subscript $i$ for brevity)
\begin{align}\label{eqn:steering_vector}
    \textbf{a}(\theta,\phi) = \begin{bmatrix} e^{(\frac{2\pi\rho_k\sqrt{-1}}{\lambda}\sin\theta \sin\xi_k cos(\phi-\varphi_k)+\cos\xi_k\cos\theta)}\\ \vdots \\  e^{(\frac{2\pi\rho_l\sqrt{-1}}{\lambda}\sin\theta \sin\xi_l cos(\phi-\varphi_l)+\cos\xi_l\cos\theta)}\end{bmatrix}
\end{align}
%(($x_i(t)$, $y_i(t)$, $z_i(t)$) in euclidean coordinates)

\noindent As $\mathbf{h_{ij}(t)}$ is a vector of signal measurements at each position in $\boldmath{\chi_i}\textbf{(t)}$, the steering vector enables calculating the phase difference between antenna positions in virtual antenna array, which then can be used with AOA calculation algorithms like Bartlett to obtain $F_{ij}(\phi,\theta)$ for pair of communicating robots $i$,$j$. 

However, since the wireless signal transmitter and receiver are separate Wi-Fi devices (i.e. different robots in a team), the signal oscillators in those devices have different frequencies with offset $\Delta_f$. This leads to time-varying phase offset in the signal phase called \emph{Carrier Frequency Offset} (CFO), leading to erroneous measurements. Following the development in~\citep{Gil2015AdaptiveCI}, we use~\emph{channel reciprocity} to rectify this. Channel reciprocity states that i) ratio of forward and reverse channel (See Fig.~\ref{fig:foward_reverse}) is constant over time i.e $h_{ij}(t)/h^r_{ij}(t)=\kappa_h$, where $\kappa_h$ is constant because the forward and backward channel would be received almost simultaneously and ii) The frequency offset in reverse direction is the negative for offset in forward direction i.e - $\Delta_f$. Hence, the observed forward and reverse channels, $\hat{h}_{ij}(t)$ and $\hat{h}^r_{ij}(t)$ respectively, that are affected by frequency offset $\Delta_f$ (and -$\Delta_f$), are given as follows for any position $p_i(t)$ in the sub-trajectory:
\begin{align}
    \label{eqn:forward_backward_channel}
    \hat{h}_{ij}(t) = h_{ij}(t)e^{-2\pi\Delta_f(t-t_k)} \\
    \hat{h}^r_{ij}(t) = h_{ij}^r(t)e^{2\pi\Delta_f(t-t_k)}
\end{align}
%\textcolor{red}{NOTE: why does the above eqn use $t_k$? Should be $t$ perhaps?}
% \edit{We use the MUSIC algorithm~\citep{Gil2015Spoof-Resilient} to derive the AOA profile to a source robot $j$ from robot $i$ as:
% \begin{equation}
% \label{eq:fij}
% F_{ij}(\theta,\phi)=\frac{1}{\left|Eig_n(h({(t_k)}\hat{h}(t_k))e^{2}a(\theta,\phi)\right|^2}
% \end{equation}}
\noindent We then obtain the rectified wireless channel $h_{ij}(t)$ as the product of observed forward channel $\hat{h}_{ij}(t)$ and reverse channel $\hat{h}^r_{ij}(t)$: 
\begin{align}\label{channel_forward_revese_prod}
    h_{ij}(t) = \sqrt{\hat{h}_{ij}(t)~\hat{h}^r_{ij}(t)/\kappa_h}
\end{align}
%(\textcolor{red}{can we explain here about $\lambda/4$?, since we don't take the square root of the channel?}).

\noindent Rewriting Eqn. \ref{eqn:bartlett_estimator} and dropping $\kappa_h$ as it is a constant scaling factor, we get the AOA profile of transmitting robot $j$ for a receiving robot $i$ as follows:
\begin{equation}
    \label{eqn:bartlett_estimator_fin}
    F_{ij}(\phi,\theta)={\left|\sum_{t=t_k}^{t_l} \hat{h}_{ij}(t)~\hat{h_r}_{ij}(t)~\text{a}(\theta,\phi)(t)\right|^2}
\end{equation}
% \edit{We use the MUSIC algorithm~\citep{Gil2015Spoof-Resilient} to derive the AOA profile to a source robot $j$ from robot $i$ as:
% \begin{equation}
% \label{eq:fij}
% F_{ij}(\theta,\phi)=\frac{1}{\left|Eig_n(h({(t_k)}\hat{h}(t_k))e^{2}a(\theta,\phi)\right|^2}
% \end{equation}}
% \noindent where \edit{${F_ij(\theta,\phi)}$ is calculated for all possible pairs of $(\theta,\phi)$ and constitutes our \emph{AoA profile} and is maximized for true signal direction $(\hat{\theta},\hat{\phi})$ which is our AoA} (\edit{How do we distinguish between strongest signal direction and true direction here?}).
%==============moving ends schematic=============
\begin{figure}
    \centering
    \includegraphics[width=7.7cm,height=6.7cm]{Images/Moving_ends_schematic.PNG}
	\caption{\footnotesize{\emph{Schematic showing relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ of the UAV with respect to moving transmitting ground robot $j$. $\boldmath{\chi_i}\textbf{(t)}$ and $\boldmath{\chi_j}\textbf{(t)}$ denote the actual trajectories of the robot $i$ (emulating virtual antenna array) and robot $j$.}}}
	\label{fig:Moving_ends_schematic}
\end{figure}
%==============moving ends schematic=============

This formulation provides the solution to the problem of measuring $F_{ij}(\phi,\theta)$ over arbitrary robot trajectories in 3D space for the static transmitting robot case. Thus by allowing robots to emulate an antenna array in full 3D space over its local trajectory, we obtain maximum magnitude signal path $AOA_{max}$ to a static neighboring robot. We address the more general problem of simultaneous mobility of both the transmitting and receiving robot, the \emph{moving ends problem}, in the subsequent section.


==> text/background.tex <==
\section{Background and Notation}
In this section we present important notational conventions used as well as essential background on wireless signals and Synthetic Aperture Radar (SAR) that we will use throughout. 
\vspace{-14pt}
\subsection{Coordinate system}\label{notation_coordinate_system} As our system returns angular information, we formulate our problem in a spherical coordinate system. Fig.~\ref{fig:3DcoordinateSystem} shows a schematic representation of a robot trajectory and it's local spherical coordinate system. $\varphi$ and $\xi$ are the azimuth and elevation angles of the receiving robot $i$ at a given position along it's trajectory. The AOA tuple ($\phi$, $\theta$) represents the transmitting robot's relative azimuth and elevation direction with respect to the initial position (at time $t_k$) of robot $i$. $\phi$ and $\varphi$ are measured counter-clockwise from the x-axis while $\theta$ and $\xi$ are measured clockwise from z-axis. Robot $i$'s position at time $t$ denoted by $p_i(t)$, is represented as ($\rho_i(t)$,$\varphi_i(t)$,$\xi_i(t)$). In the case that the robot trajectory is obtained via on-board sensors or estimation techniques the positions are denoted by $\hat{p_i}(t)$. This position measurement is subject to error which we denote as $\kappa_{\rho}$, $\kappa_{\phi}$ and $\kappa_{\theta}$ for errors in $\rho$, $\varphi$, $\xi$ respectively. We denote estimated relative AOA (from our system) between robots $i$ and $j$ as $(\hat{\phi},\hat{\theta})$ and the true AOA (from motion capture system) as $(\phi_g,\theta_g)$. Our experimental evaluation uses Cartesian coordinates for robot's position, represented as ($x_i(t)$, $y_i(t)$, $z_i(t)$).\footnote{A position ($\rho$,$\phi$,$\theta$) in spherical coordinates has corresponding Cartesian coordinates ($x,y,z$) as ($\rho\sin\theta\cos\phi, \rho\sin\theta\sin\phi, \rho\cos\theta$).}
% \subsection{Robot Trajectory.}   For a robot $i$, let it's pose at time $t_{k}$ be $\bold{\chi}_i(t_{k}) = (R_i(t_k)R_{\epsilon}(t_k), p_i(t_k)+p_{\epsilon}(t_k))$, where $R_i(t_{k}) \in SO(3)$ is orientation, $p_i(t_k) \in \mathbb{R}^3$ is position. We define a local sub-trajectory of the robot over which we intend to perform AOA estimation, as the trajectory of positions corresponding to $t\in[t_k,\hdots,t_l]$ as shown in Fig.~\ref{fig:3DcoordinateSystem} and we assume that this sub-trajectory is at least $2\lambda$ in length (i.e. 12cm for 5Ghz WiFi). Define this local trajectory as $\boldmath{\chi_i}\textbf{(t)}$, namely, the vector of all poses $\chi_i(t)$ for $t\in[t_k,\hdots,t_l]$, where k any timestep when the robot wants to initiate data collection for 3D SAR; i.e. to obtain relative AOA to any transmitting robots $j\in\mathcal{N}_i$ in its neighborhood, where \emph{neighborhood} $\mathcal{N}_i$ denotes any robot $j$ for which $i$ can hear ping packets (i.e. communication at the lowest rate of 6Mb/s). Note that signal packets collected over a single local trajectory $\bold{\chi}_i(t_{k})$ can be used to compute AOA profiles for \emph{all} robots simultaneously for which robot $i$ is receiving communication ping packets (not just one neighbor).
\subsection{Robot trajectory}\label{notation_robot_trajectory} For our experiments, robot positions are generally collected via trajectory estimation techniques using on-board sensors or from external motion capture system (groundtruth). We define a groundtruth local \emph{sub-trajectory} $\boldmath{\chi_i}\textbf{(t)}$ of the robot $i$ over which we intend to perform AOA estimation, as the trajectory of positions corresponding to $t\in[t_k,\hdots,t_l]$ as shown in Fig.~\ref{fig:3DcoordinateSystem}. An estimated trajectory is denoted as $\boldmath{\hat{\chi_i}}\textbf{(t)}$. We assume that sub-trajectories are \emph{local} i.e they could be as small as 12cm of total robot displacement. This comes from the known result in antenna array theory stating that a full AOA profile is attainable over a minimum array length of $2\lambda$, which is on the order of 12cm of total robot displacement for 5Ghz WiFi. 
%========Spherical coordinate system=======
\begin{figure}
  \centering
  \includegraphics[width=8.0cm,height=8.0cm]{Images/Spherical_coordinates_schematic_3.PNG}%
  \caption{\footnotesize{\emph{Spherical coordinate system used by our system in receiving robot $i$'s local frame of reference. Robot $i$ uses M wireless signal measurements and its corresponding position estimates $p(t)$ = ($\rho$,$\varphi$,$\xi$) from time $t_{k}$ to $t_{l}$, l = k + M for each position (red antennas) to emulate M virtual antenna array elements and obtain relative angles $\phi$ (azimuth) and $\theta$ (elevation) to the signal transmitting robot $j$. True relative AOA (obtained from motion capture system) is denoted by $(\phi_g, \theta_g)$.}}}
  \label{fig:3DcoordinateSystem}
\end{figure}
%========Spherical coordinate system======

$\boldmath{\chi_i}\textbf{(t)}$ is the vector of all poses $\chi_i(t_{k}) = (R_i(t_k), p_i(t_k))$ for $t\in[t_k,\hdots,t_l]$, where $R_i(t_{k}) \in SO(3)$ is orientation, $p_i(t_k) \in \mathbb{R}^3$ is position. $k$ is any timestep when the robot wants to initiate data collection for 3D SAR; i.e. to obtain relative AOA to any transmitting robots $j\in\mathcal{N}_i$ in its \emph{neighborhood}. $\mathcal{N}_i$ includes all transmitting robots $j$ for which robot $i$ can atleast obtain ping packets (i.e. broadcasting at 5 kB/s over 3 seconds). Note that signal packets from all $j\in\mathcal{N}_i$ simultaneously collected over a single local trajectory $\boldmath{\chi_i}\textbf{(t)}$, can be used to compute individual AOA profiles for \emph{all} robots in parallel. A pose of robot $i$ in $\boldmath{\hat{\chi_i}}\textbf{(t)}$ at time $t_{k}$ is represented as $\hat{\chi_i}(t_{k}) = (R_i(t_k)R_{\epsilon}(t_k), p_i(t_k)+p_{\epsilon}(t_k))$. Let $R_{\epsilon}(t)$ and $p_{\epsilon}(t)$ denote the accumulated error in estimated position and orientation from time $t_0$ (The very first timestep when robot start to move) to any time $t_k$.

We use $\hat{p_i}(t)$ to denote robot $i$'s estimated position for a pose in $\boldmath{\hat{\chi_i}}\textbf{(t)}$ i.e $\hat{p_i}(t)$ = $p_i(t_k)+p_{\epsilon}(t_k)$. As our system can handle the motion of transmitting robots, let $\boldmath{\chi_{ij}}{(t_{k:l})}$ denote the relative trajectory of robot $i$ with respect to another robot $j\in\mathcal{N}_i$ over the time window from $t=t_k$ to $t=t_l$, calculated as $\boldmath{\chi_{ij}}{(t_{k:l})}$ = $\boldmath{\chi_i}{(t_{k:l})}$ - $\boldmath{\chi_{j}}{(t_{k:l})}$. For brevity we denote this \emph{relative} sub-trajectory over the time vector $[t_k,\hdots,t_l]$ as $\boldmath{\chi_{ij}}\textbf{(t)}$ in the sequel. In Sec. \ref{sec:moving_ends} we show its validity even when the coordinate frames of robot are different. 

\subsection{A primer on Synthetic Aperture Radar (SAR).}\label{notation_SAR} An application of SAR over robot trajectories requires that a robot travel over some small local displacement (of at least $2\lambda$) while taking several measurements $h_{ij}(t)$ of the wireless communication channel from its neighboring robots $j\in\mathcal{N}_i$. The ideal channel at time $t$ is modeled following the common far-distance assumption when signal waves are assumed to be planar \citep{Tse2005FundamentalsOW} :

\begin{align}\label{eqn:channel_basic_eqn}
    h_{ij}(t) = \frac{1}{d_{ij}(t)}e^{(\frac{-2\pi\sqrt{-1}}{\lambda}d_{ij}(t))}
\end{align}
\noindent where $d_{ij}(t)$ is the groundtruth distance between $p_i(t)$ and $p_j(t)$. Over its trajectory, the robot creates a history of packet-position tuples $<h_{ij}(t),p_i(t)>$, where each such tuple is essentially an emulation of omnidirectional ``antenna element'' in a virtual multi-antenna array. In the case of WiFi pings or thousands of packets can be transmitted at 5kB/s which is much lower than the lowest protocol rate of 6Mb/s, a large number of antennas can be emulated with very little communication overhead\footnote{The total communication overhead incurred by our system is around 15 Kb}. Thus using its local trajectory and transmitted signals from robot $j\in\mathcal{N}_i$, the wireless channel at robot $i$ can be modeled using the multi-antenna array output observation model from~\citep{Vu2010PerformanceAO} as: 

\begin{equation}\label{eq:array_model}
    \mathbf{Y_{ij}(t)}=[Y(t_k),\hdots,Y(t_l)]^T=\mathbf{a}(\theta,\phi)\mathbf{(t)}\mathbf{h_{ij}(t)}+\mathbf{n(t)}
\end{equation}
%=========3D SAR profile=======
\begin{figure*}
\centering
  \includegraphics[width=15.3cm,height=6.5cm]{Images/AOA_using_3D_SAR_v2.png}
  \caption{\footnotesize{\emph{(a) Shows the arbitrary 3D groundtruth trajectory of a signal receiving UAV from our hardware experiments, the start position $p(t_k)$ indicated by a blue circle. (b) Corresponding AOA profile obtained for the trajectory using our formulation shows the \emph{AOA} (strongest signal direction) which corresponds to the relative direction of the transmitting robot (indicated by black antenna) located at true AOA ($\phi_g$, $\theta_g$) = ( $\ang{-90}$, $\ang{91}$) and at a distance of 10 m in line-of-sight. Our system returns AOA ( $\hat{\phi}$, $\hat{\theta}$) = ( $\ang{-91.5}$, $\ang{92.5}$).}}}
  \label{fig:3D_SAR_AOA}
\end{figure*}
%=========3D SAR profile=======

\noindent where $Y(t_k)$ is received signal at robot position $p_i(t_k)$, the total number of signal packets received is $M$, and $l=k+M$. The vector $\textbf{a}(\theta,\phi)\textbf{(t)}$ is the \emph{steering vector}, which is defined by the robot's local trajectory $\boldmath{\chi_i}\textbf{(t)}$ and thus dictates the \emph{geometry} of arbitrary 3D antenna array. This steering vector is a function of the geometry of the antenna array (i.e. robot $i$'s positions $p_i(t)$, $t\in[t_k,t_l]$ ) and the angle tuple ($\phi$, $\theta$) for transmitting robot $j\in\mathcal{N}_i$ (See Fig. \ref{fig:3DcoordinateSystem}):
\begin{align}\label{eqn:steering_vector_eqn_basic}
    \textbf{a}(\theta,\phi)\textbf{(t)} = e^{(\frac{2\pi\sqrt{-1}}{\lambda}f(p_i({t}), \phi, \theta))}
\end{align}

\noindent Here, $\lambda$ is the signal wavelength and $\textbf{n({t)}}$ is a signal noise vector, assumed to be Gaussian, circular, independent and identically distributed, with a mean of zero and a covariance of $\sigma^2I$, where $I$ is the identity matrix of appropriate dimension. The wireless channel measurement at time $t$, $h_{ij}(t)$, which is a complex number capturing the phase and magnitude of the received signal, can be obtained using the \emph{Channel State Information (CSI) Toolbox} \citep{Halperin_csitool}. $\mathbf{h_{ij}(t)}$ = $[h_{ij}(t_k),\hdots,h_{ij}(t_l)]$ is thus known at the receiving robot. 

Using direction finding algorithms like Bartlett or MUSIC from antenna array theory~\citep{Krim1996TwoDO}, the AOA profile ${F_{ij}(\phi,\theta)}$ can be obtained by measuring the signal phase difference of each array element with respect to the first element at $p(t_k)$. We use the Bartlett estimator we get:

\begin{equation}
    \label{eqn:bartlett_estimator}
    F_{ij}(\phi,\theta)=%{\left|\sum_{t} \textbf{h_{ij}(t)}*\textbf{a}(\theta,\phi)\textbf{(t)}\right|^2}
    {\left|\sum_{t=t_k}^{t_l} {h_{ij}(t)}~a(\theta,\phi)(t) \right|^2}
\end{equation}

\noindent ${F_{ij}(\phi,\theta)}$ thus refers to relative paths a WiFi signal traverses between a given pair of signal transmitting robot $j$ and receiving robot $i$. Mathematically, it is a 2D matrix calculated for all possible incoming signal directions along azimuth and elevation (360 x 180). 
%We note that our system can be easily accommodate the simultaneous generation of AOA profiles simultaneously multiple transmitting robots as their received signals can be filtered by mac address at the receiver robot. 
Thus, henceforth we refer to $AOA_{max}$ as the strongest signal direction $(\hat{\phi},\hat{\theta})$, or \emph{ the AOA peak corresponding to maximum magnitude path}, in the full AOA profile $F_{ij}(\phi,\theta)$. 
%This needs to be discussed based on changes in the problem statement
%\textcolor{red}{We denote by ($\Tilde{\phi},\Tilde{\theta}$), the incorrect estimation of AOA due to errors introduced on account of trajectory estimation.}

\medskip
\noindent A reference to all notations and terminology can be found in Appendix section \ref{sec:notations}. Next we formulate the problems that are addressed in this paper.

==> text/conclusion.tex <==
\section{Discussion} \label{sec:discussion}
% In this paper we have developed a method for robots to ``sense'' relative spatial information for all of their neighboring robots with whom they minimally communicate.  Specifically, we develop a method for acquiring rich directional signal profiles, capturing all of the paths that a signal traverses through the environment when communication occurs between any two robots. Understanding this information with characterizable accuracy as we do in this paper, opens the door to sensing many important quantities. For example, it has been shown that such profiles can be used for detecting the uniqueness of the sender, thereby better securing several multi-robot coordination tasks against spoofing or (Sybil) attacks \citep{Gil2015Spoof-Resilient}. To our knowledge, this is the first paper to develop directional signal sensing in a way that is truly compatible to general robotic platforms, by relaxing constraints on motion. 
In this discussion section we address some practical considerations that need to be taken into account when integrating this system with robot platforms in its current form as well as avenues of improvement and future work. 

\subsection*{Practical considerations}
Here we address some practical considerations of our work stemming from factors that arise in implementation. We note that discretization of the virtual antenna array elements resulting from a combined effect of trajectory estimation errors and significant WiFi packet loss during transmission, is possible in some implementations. We leave this analysis as an avenue for investigation in future work and in this paper assume that the loss in packet transmission is not severe.  For implementation scenarios, a future version of the work could include control of packet transmission as well as optimization of robot trajectories to diminish the occurrence and potential impact of discretization effects.
%=======Future Work stats============
\begin{figure}
    \centering
    \includegraphics[width=7.5cm,height=6.7cm]{Images/Future_work_manipulator_arm_3.PNG}
	\caption{\footnotesize{\emph{Hardware experiment showing a proof-of-concept where an AOA profile is obtained from arbitrary 3D motion of a manipulator arm using the methodologies presented in this paper. Here, a WiFi patch antenna was adhered to the manipulator at the end of the robot arm and ping packets from a second manipulator arm were collected for AOA profile generation.  Due to very low estimation error in the trajectory, the resulting AOA profile demonstrates a very clear and almost zero noise peak along the direct path between the two manipulators.}}}
	\label{fig:future_work_manipulator_arm}
\end{figure}
%=======Future Work stats============
\subsection*{Future work}
Here, we summarize a few directions of interesting future work that could build upon our developed framework and accompanying analysis. Namely we discuss 1) using the measure of informativeness of robot trajectories for \emph{optimization} purposes, 2) the application of our developed framework to collaborative robot perception tasks such as multi-robot mapping and 3) the potential impact of our work on other robotics tasks, including seemingly disparate tasks such as improving manipulation with a robot arm. 

\paragraph{Optimizing informativeness:} This paper develops the concept of \emph{informativeness} of different robot trajectories for the purpose of obtaining AOA profiles $F_{ij}(\phi,\theta)$ between robots. Interesting avenues of future investigation could include studying the trade-offs between different levels of informativeness and the modification of the robot's natural motion, i.e. co-optimizing the robot trajectories to improve informativeness while achieving their primary coordination task. Additionally using relative trajectories could naturally lead to more informativeness as seen in Sec. \ref{sec:results_movingEnds}.

\paragraph{Multi-robot perception:} The algorithmic framework and analysis presented in this paper addresses sensing over each individual communication link between pairs of robots. One can use this as a basis for \emph{multi-robot} perception where sensed directional profiles can be shared with neighboring robots to achieve several interesting capabilities such as positioning for the entire team, multi-robot mapping without the need for a common reference frame, and/or performing sensor fusion of this information with other more traditional on board sensors such as cameras or LiDARs to learn about the environment. 

\paragraph{Robot manipulation:} One perhaps surprising outcome of our work on generalizing SAR capabilities to arbitrary 3D robot trajectories, is the applicability of this method to seemingly very different robotic platforms such as robot manipulator arms, that also traverse 3D space along arbitrary trajectories. In fact for these systems, the arbitrary 3D SAR development from this paper can be applied fruitfully, taking advantage of the fact that the manipulator position in 3D space can be estimated to very high precision using inverse kinematics. Here, a small patch WiFi antenna can be mounted on the tip of the manipulator and used to measure multipath profiles generated by passing WiFi signals through objects in the workspace (such as a closed container), or these profiles can be used to measure the relative direction to another manipulator arm or mobile base for enhanced collaboration abilities. The analysis on informative trajectories developed in this paper can be used to co-optimize manipulator arm motion for enhancing attainable $F_{ij}(\phi,\theta)$, as the manipulator achieves its primary task, such as approaching or manipulating an object.  


% Our focus has been to introduce the commodity WiFi module as a new on-board sensor in order expand the portfolio of sensing modalities available for robots. This opens up interesting research avenues that can potentially improve the accuracy of the acquired information even further. As the sensor leverages robot's motion, trajectory error is one of the major factors that impact AOA estimation as shown in our analysis. If the robot can estimate it's trajectory errors to some extent, then incorporating that in the steering vector given in equation (\ref{eqn:steering_vector}) could potentially improve AOA accuracy. A detailed analysis of the impact of these factors (i.e trajectory error, intrapose spacing etc) specifically for non line-of-sight scenarios would help to optimize AOA estimation with signal multipaths. Although we characterize the \emph{informativeness} of different shaped trajectory, the effect of such distorted  emulated antenna arrays on AOA estimation has not been looked into. From an implementation perspective, there are several aspects of this research that can be further improved upon. Development of a framework for AOA calculation with on-board device would enable to an independent deployment and is being actively pursued as part of our next steps. 

\section{Conclusion}
\label{sec:conclusion}
In this paper we develop a system that enables a robot to use local information to obtain spatial information of all other robots on its team with which it can exchange ping packets. Our key idea is to exploit estimated robot trajectories to trace virtual 3D antenna arrays for attaining \emph{continuous} AOA profile generation even in the presence of robot motion at both ends (receiving and transmitting robots). We provide a full theoretical analysis, supported by in-depth experiments, for understanding the informativeness of different robot paths for extracting maximum magnitude path $AOA_{max}$ in the AOA profile from the communication signals, as well as the impact of trajectory estimation error on $AOA_{max}$ accuracy. To our knowledge, this is the most general implementation of such a capability to date. Specifically, our framework is compatible with multi-robot systems that are mobile in 2D and 3D space, are heterogeneous, and must coordinate in potentially cluttered environments with large inter-robot distances as shown by our experimental results and application study.

==> text/impact_factors_lemmas.tex <==
\subsection{Characterizing the impact of trajectory estimation error on Angle-of-Arrival estimation}
\label{sec:characterization-trajectory-err-analysis}
% \edit{Our goal is to characterize the effect of trajectory estimation error on computing our Angle-of-Arrival profile. With all on-board sensing on our robot platforms we expect some amount of error in our robot trajectory estimates which corresponds to an error in antenna geometry or the steering vector. (The effect of this error may be similar to a calibration error for antenna arrays?).}

As an implementation of SAR requires knowledge of local robot displacements (see Section~\ref{sec:Development}), one must rely on trajectory estimation techniques for robots operating in a field. Most often, robot displacements can be estimated using onboard sensors such as inertial measurement units (IMU), cameras, or LiDAR for trajectory estimation. However the error in a local trajectory $\boldmath{\hat{\chi_i}}\textbf{(t)}$ due to different estimation approaches translates into error in steering vector (incorrect antenna positions) when used for SAR. Thus, it is necessary to analyze our system's performance under cases where the measured displacement is different from groundtruth displacement. 

Since, our method requires only \emph{local} displacement (sub-trajectory) information, it is not impacted by large accumulations of errors. Specifically, for any given AOA profile calculation only the sub-trajectory of positions as indicated by $\hat{p}(t)$ from $t=[{t_{k},\hdots,t_{l}}]$ are used to emulate a virtual antenna array (See Fig.~\ref{fig:3DcoordinateSystem}); 
%this sub-trajectory length can be as small as 12 cm. 
This means that at any specific instance of 3D SAR, robot positions at timesteps not between $t_{k},\hdots,t_{l}$ are irrelevant for AOA estimation. Thus, our development here focuses on impact of $\boldmath{\hat{\chi_i}}\textbf{(t)}$ and the residual errors (Defn. \ref{def:residual_error}) accumulated over $\boldmath{\hat{\chi_i}}\textbf{(t)}$, on \emph{AOA}. Comparing the results for groundtruth and Intel Realsense T265 tracking camera trajectories from hardware experiments (Fig.~\ref{fig:Traj_comparison}) we see that higher error in the latter impacts the estimated AOA profile. Our goal in this section is to mathematically model and analyze this impact as a function of trajectory estimation error. 

We use the angular drift metric from Defn. (\ref{def:angular-drift}) to quantify the residual error in trajectory estimation for our theoretical analysis. We assume that the errors for position ($x_i(t)$, $y_i(t)$, $z_i(t)$) in Cartesian coordinates are translated to errors in $\varphi_i(t)$ and $\xi_i(t)$ only in the corresponding spherical coordinates. 
 %We then show results of a simulation study for on-board sensor trajectory that uses both angular drift and $ATE_{trans}$. 
We introduce two lemmas to show the impact of constant and varying angular drift on AOA estimation. To simplify our analysis, we use ideal circular arc trajectories in 3D and show that results for arbitrary 3D trajectories from hardware experiments closely follow our theoretical findings. 
% ii) use Bartlett equation for AOA estimation following the development in~\cite{Gil2015AdaptiveCI,Zhang2019OnTF} which, in it's general form is given as : 
% \begin{equation}
%     \label{eqn:bartlett_estimator}
%     F_{ij}(\theta,\phi)={\left|\sum_{t} h(t)\text{a}(\theta,\phi)\right|^2}
% \end{equation}
% \noindent where $h(t)$ is the wireless signal channel and $\text{a}(\theta,\phi)$ is the steering vector.} 
% \begin{case}{\emph{Co-relating error accumulation in trajectory estimates with AOA error:}}
% For a given angular error in trajectory estimation %$\Delta_{\text{traj}}$, 
% what is the error %$\Delta_F$ 
% to be expected in the AOA obtained from AOA estimation? We consider both the case of constant and varying error.
% \end{case}
% \begin{case}{\emph{Analyzing anomalous peaks in wireless signal profile due to increased inter-element separation:}}
% We wish to characterize the maximum distance between consecutive elements of the traced antenna array tolerable before anomalous peaks start dominating the wireless signal profile leading to obfuscation of true AOA peak.  
% \end{case}
%  Next we introduce three lemmas that provide the proofs for our analysis of the above cases.
%====MOcap_vs_Camera_AOA_accuracy====
\begin{figure}%===Drift accumulation=======
		\centering
        \includegraphics[width=8.0cm,height=5.5cm]{Images/Drift_accumulation_mocap_vs_camera.png}
    	\caption{\footnotesize{\emph{Hardware experiment showing the drift in Intel Realsense T265 tracking camera trajectory compared to groundtruth trajectory.The end positions points (red) are much further away from each other than the start points (green) indicating drift accumulation.}}}
    	\label{fig:drift_accumulation}
\end{figure}%===Drift accumulation=======

\subsubsection{Constant offset:}
We first analyze the case of a constant offset; for example, as would occur in the case of a bias or drift in the trajectory estimation. We use a circular 3D trajectory of radius $R$ to simplify the analysis.
\begin{lemma}
 If the measured trajectory in spherical coordinates is incorrect by a constant azimuth offset $\kappa_{\phi}$ and a constant elevation offset $\kappa_{\theta}$, the observed AOA peak will occur at a shifted angle of $\phi-\kappa_{\phi}$, $\theta-\kappa_{\theta}$.
\end{lemma}
\noindent \textit{Proof: } Assume that the transmitting robot $j$ at a point $(D,\phi,\theta)$ is very far from the receiving robot $i$'s trajectory, which is the arc of a circle of radius $R$. The distance from robot $j$ to the bottom of the trajectory arc is given by $D-R\cos\phi\cos\theta$. By rotating our coordinate system, we get $D-R\cos(\phi-\varphi(t_u))\cos(\theta-\xi(t_u))$ as the distance from robot $j$ to an arbitrary point on our arc, given robot $j$'s $(\phi,\theta)$ and virtual antenna element location $(\varphi(t_u),\xi(t_u))$ on robot $i$'s trajectory. Thus, applying the general model of the wireless channel (Eqn. \ref{eqn:channel_basic_eqn}) for a circular trajectory based on distance $D$ and radius $R$ of the receiving robot trajectory, our forward-reverse channel product at a given ($\varphi(t_u),\xi(t_u)$) is the following (dropping notation $t$ in RHS of the equation for brevity):
\begin{align}\label{eqn:forward-reverse-sim}
    &h_{ij}(t_u) = \frac{1}{D^2}e^{\frac{-4\pi\sqrt{-1}~D}{\lambda}}*e^{\frac{-4\pi\sqrt{-1}~\rho~cos(\phi-\varphi_u)cos(\theta-\xi_u)}{\lambda}}
\end{align}
Due to some constant drift $\kappa_{\phi}, \kappa_{\theta}$, however, we instead measure a peak at some angle $\hat{\phi}$ rather than at $\phi$, and some angle angle $\hat{\theta}$ rather than at $\theta$, defined from the AOA profile (cf. Eqn.~\eqref{eqn:bartlett_estimator_fin}) as follows:
\begin{align}
\begin{split}
    &F_{ij}(\phi,\theta)= \frac{1}{D^2}\sum_{u=1}^{M}e^{\frac{-4\pi\sqrt{-1}~D}{\lambda}}* \\
    &\ \ \ \ \ \ \ \hspace{-10pt}e^{\frac{-4\pi\sqrt{-1}~\rho[cos(\phi-\varphi_u)cos(\theta-\xi_u)-cos(\hat{\phi}-\varphi_u+\kappa_{\phi})cos(\hat{\theta}-\xi_u+\kappa_{\theta})]}{\lambda}}
    \label{eqn:beta}
\end{split}
\end{align}
% We further simplify this to:
% \begin{equation}
%     P(\beta)= A\sum_{i-1}^{n}e^{-j4\pi~r[sin(\frac{\alpha-\beta+\Delta}{2})sin(\frac{\alpha+\beta-2\phi-\Delta)}{2}]}
% \label{eqn:beta}
% \end{equation}
% Where $k=\frac{-j4\pi~r}{\lambda}$.
This takes the form of the well-known Bessel function, which is maximized at $\hat{\phi}=\phi-\kappa_{\phi}$ and $\hat{\theta}=\theta-\kappa_{\theta}$~\citep{circularAntennaArrays}.

\subsubsection{Varying offset:}
Beyond constant offsets such as drift or bias, other errors that may complicate our analysis include the vibrations of drones and time-varying drifts in trajectory across narrow data-capture windows. Our following analysis considers the effect of this varying offset (Fig. \ref{fig:drift_accumulation}).
\begin{lemma}
\label{lemma:trajError}
For a measured trajectory incorrect by some average offset $\kappa_{\phi}$ with a max deviation of $\delta$ around $\kappa_{\phi}$ in the azimuth direction, and some average offset $\kappa_{\theta}$ with a max deviation of $\mu$ around $\kappa_{\theta}$, there will exist a peak located at angle $(\phi-\kappa_{\phi}, \theta-\kappa_{\theta})$, in line-of-sight conditions. This peak will attenuated by a factor no more than $cos(\frac{\delta+\mu}{2})$, relative to the peak in absence of trajectory offsets.
\end{lemma}

%\textcolor{red}{SG:The notation below in the proof for Lemma 3 versus Lemma 2 seems to change a lot and makes it difficult to follow. How do $\alpha$ and $\beta$ relate to $\phi$ and $\theta$ from Lemma 1? what about $\delta_i$ and $\mu_i$? Do they relate to $\kappa_\phi$ and $\kappa_\theta$? If so, how?  This is not explained currently and so it is easy to lose the thread going from Lemma 2 to Lemma 3.  Also what does the counter $i$ indicate here? Is it still ``antenna element''?}
\noindent \textit{Proof: }  We consider the \emph{phase} component $\angle F(\phi, \theta)$ of Equation \ref{eqn:beta} (in the exponent) from the previous lemma, substitute a= $\phi-\varphi_u$ and b= $\theta-\xi_u$ and modify it for a varying $\kappa_{\phi}$ and $\kappa_{\theta},$ indicated by subtracting deviations from the mean for each position, $\delta_u, \mu_u$:
\begin{equation}
\begin{split}
    &\hspace{-0.1in}\angle\textit{F}(\phi, \theta)= \\ &\hspace{-0.1in}\frac{-4\rho\pi\sqrt{-1}}{\lambda}[cos(a)cos(b)-cos(a-\delta_u)cos(b-\mu_u)]
\end{split}
\end{equation}

\noindent Assuming $\delta_u$ and $\mu_u$ are relatively small, we can simplify our equation using trigonometric identities to the following:
\begin{equation}
\begin{split}
     &\hspace{-0.1in}\angle \textit{F}(\phi,\theta)=\\
     &\hspace{-0.1in}\frac{-4\rho\pi\sqrt{-1}}{\lambda}[\delta_u~sin(a)cos(b)+\mu_u~sin(b)cos(a)]
\end{split}
\end{equation}

\noindent Consider the worst-case scenario, where $\delta=\delta_{max}$ and $\mu=\mu_{max}$, and $\delta=-\delta_{max}$ and $\mu=-\mu_{max}$, alternately. For brevity, we represent the quantity $\frac{1}{D^2}e^{\frac{-4D\pi\sqrt{-1}}{\lambda}}$ with $\alpha$, and group these alternate phases together (thus changing the bounds of our summation). We can rewrite our profile as follows:
\begin{equation*}
    F_{ij}(\phi,\theta)\geq~\alpha\sum_{u=1}^{M/2}e^{\frac{\sqrt{-1}~(\delta_{max}+\mu_{max})}{2}}+e^{\frac{-\sqrt{-1}~(\delta_{max}-\mu_{max})}{2}}
\end{equation*}
\begin{equation}
    \text{i.e.}~F_{ij}(\phi,\theta)\geq~\alpha M cos{\frac{\delta_{max}+\mu_{max}}{2}}
\end{equation}
\noindent Thus, our peak at $\phi-\kappa_{\phi}$, $\theta-\kappa_{\theta}$ from Lemma 1 is attenuated by a factor that is at most $cos\frac{\delta_{max}+\mu_{max}}{2}$ vs. the peak in the absence of drift.
% %===Antenna Spacing figure============
% \begin{figure}
%     \centering
%     \includegraphics[width=9.5cm]{Images/NgNbGraphic.jpg}
% 	\caption{\footnotesize{\emph{Schematic for SAR array reconstruction of a robot trajectory. The well-space antenna elements have an inter-element distance less than $\frac{\lambda}{4}$ while the poorly-spaced antennas violate that threshold.}}}
% 	\label{fig:antenna_spacing}
% \end{figure} 
% %===Antenna Spacing figure============

Our hardware experiment results bolster these theoretical findings. A representative trace is shown in Fig.~\ref{fig:Traj_comparison}, which provides comparison between two wireless signal profiles using motion capture versus a tracking camera. The side view for the profiles indicates an attenuation of the maximum AOA peak as expected from the analysis of this section. From a top view  the predicted peak shift can also be seen for the trajectory estimation case (``using Noisy Estimated Trajectory'' case) versus the case where motion capture is used to provide the trajectory estimate. 

Section~\ref{sec:results_traj_erro_AOA} demonstrates aggregate results showing the impact of trajectory estimation error on AOA error on average, where robot trajectories are estimated using an Intel RealSense T265 tracking camera. It also includes results for a simulation study demonstrating the relationship between increasing trajectory estimation error and AOA estimation error (see Fig.~\ref{fig:aoa_vs_ATE_error}).
% Section~\ref{sec:results_traj_erro_AOA} also includes results for a simulation study demonstrating the relationship between increasing trajectory estimation error (measured as yaw error of the robot) and AOA estimation error (see Fig.~\ref{fig:Aggregate_AOA_error_vs_mean_yaw}).

% %====Bad antenna elements==
% \begin{figure}
% 		\centering
%         \includegraphics[width=7.5cm,height=5.5cm]{Images/Bad_element_percent_allOnBoard.png}
%     	\caption{\footnotesize{\emph{Percentage of poorly-spaced antenna elements (antenna element spacing greater than discretization threshold of $\lambda$/4) for a total of 59 on-board sensor trajectories. A majority of trajectories have violations between 10\% to 20\% }}}
%     	\label{fig:Bad_element_percent_allOnBoard}
% \end{figure}
% %===Bad antenna elements======= 
% \subsection{Trajectory Discretization}
% \label{sec:Trajectory_discretization} Here we analyze the impact of antenna element spacing of the virtual antenna array, on AOA profile. Essentially we want to understand at what point the "anomalous peaks" in AOA profile dominate the "main-peak" (that corresponds to strongest signal direction). Firstly, we consider a simplified 2D circular trajectory so as to isolate the impact of discretization from trajectory geometry. We provide numerical analysis of how an increase in separation of antenna array elements for such trajectory geometry, results in dominating anomalous peaks.
% Next, we provide a general formulation that compares the correct AOA peak in AOA profile with anomalous peaks, given that a trajectory of arbitrary shape has \emph{good elements} (well-spaced positions of emulated antenna array) and \emph{bad elements} (poorly-spaced positions of emulated antenna array) - Fig.~\ref{fig:antenna_spacing}. Poorly-spaced positions refer to those positions in the trajectory which violate a specific discretization threshold (Fig.~\ref{fig:Bad_element_percent_allOnBoard}).

% \subsubsection{Analysis of spacing for 2D antenna array.}\label{sec:discretization_2D_array}
% We analyze the special case of 2D circular antenna array and provide results from numerical analysis of the derived formulation. Following the developments in~\cite{circularAntennaArrays} (Section 3.2.2) the excitation of an circular antenna array with radius $r$, phase mode $m$ and $M$ antenna elements is given as:
% \begin{align}
%     \label{eqn:array_excitation_2D}
%     f_m^s(\zeta,\phi)=\frac{1}{M}\sum_{n=0}^{M-1}e^{jm\gamma_n}e^{j\zeta\cos(\phi-\gamma_n)}
% \end{align}
% \noindent where $\zeta$ = $\frac{2\pi}{\lambda}rsin\theta$. \edit{Relevant to our analysis, we set mode $m$ = 0 and $\theta$ = \ang{90} (source is in the same plane as the trajectory).} Multiplying Eqn.~\ref{eqn:array_excitation_2D} with the channel equation for a circular array as given in \cite[Section 2]{Kumar2014AccurateIL} we can rewrite Eqn. \ref{eqn:bartlett_estimator} for circular antenna array as follows :
% \begin{equation}
%     \label{eqn:main_term_subTerm_bartlett form}
%     F(\phi,\theta)=\frac{e^{\frac{-j2\pi D}{\lambda}}}{DM}\sum_{n=0}^{M-1}e^{j\zeta(\cos(\phi-\varphi_n)-cos(\hat{\phi}-\varphi_n))}
% \end{equation}
% where distance to signal transmitter $D$ = 10 m for our theoretical analysis. We can then separate the desired response (correct AOA peak) and the anomalous peaks (see Fig.~\ref{fig:Inter_element_spacing_numerical_results}) using a Fourier series expansion ~\cite[appendix A]{circularAntennaArrays} as follows:
% \begin{equation}
%     \label{eqn:main_term_separate}
%     \begin{split}
%     F(\phi,\theta) = \kappa \int_{0}^{2\pi} e^{j\zeta(\cos(\phi-\varphi_n)-cos(\hat{\phi}-\varphi_n))} d\varphi \\  + \hspace{0.1cm} \kappa\hspace{-0.2cm}\sum_{q=-\infty,q\neq0}^{\infty}\int_{0}^{2\pi}e^{j(\zeta(\cos(\phi-\varphi_n)-cos(\hat{\phi}-\varphi_n)) + qN\varphi)} d\varphi
%     \end{split}
% \end{equation}
% where $\kappa$ = $\frac{e^{\frac{-j2\pi D}{\lambda}}}{DM}$. The first term in corresponds to the desired AOA peak "main-term" while the second term corresponds to anomalous peaks. Numerical analysis of Eqn.~\ref{eqn:main_term_separate} shows that the desired threshold for inter-element spacing for an ideal 2D array geometry, so that the anomalous terms do not dominate the wireless signal profile, is $\frac{\lambda}{2}$, where $\lambda$ is the wavelength. Additional details are discussed in section~\ref{sec:discretization_impact_results}. \edit{Note that since real wireless signal require cancelling the phase offsets using the product of forward-reverse channel, the threshold is $\frac{\lambda}{4}$ \textbf{NEED CITATION}}.  
% % \begin{itemize}
% %     \item Is this the correct way of thinking about Equation~\eqref{eq:question}?
% %     \item Can we use this equation to find the point at which residual terms accumulate sufficiently so as to overtake the dominant peak (compare to the attenuated peak height in Diana's analysis)?
% %     \item It is still left to treat the error $e$ in antenna geometry which is different than antenna spacing and grating lobes however.  Perhaps the paper~\cite{luo} can help us with this objective.
% % \end{itemize}
% % }
 
% % \subsection{Informativeness: Trajectory Type versus Error in AOA}
% % As show in Figu1D trajectories have up-down, left-right ambiguity, 2D trajectories have up-down ambiguity. 3D resolve all ambiguities

% \subsubsection{General formulation for inter-element spacing:} \label{sec:general_formulation_spacing}
% As our system can result in anomalous peaks, if the combination of mobility and gaps in WiFi packet reception result in \edit{inter-element spacing larger than $\frac{\lambda}{4}$} (where $\lambda$ is the wavelength of the signal).we analyze this impact as follows:

% \begin{lemma}
% The ratio of the power at some true AOA peak $i$, $P_i(\phi,\theta)$, to the power at anomalous i.e false AOA peak $y$, $P_y$, is greater than or equal to the square of the number of well-spaced elements, $n_g$, over the square of the number of the poorly-spaced elements, $n_b$.
% \end{lemma}

% \noindent \textit{Proof: } We assume the worst-case scenario where all poorly spaced elements (indicated in blue in fig. \ref{fig:antenna_spacing}) have phases that all add up at some false peak $y$. The true peak, at $x$, will occur as a maximum in the Bartlett power profile for the well-spaced antennas. Thus, the power at $x$ can be expressed as follows \textcolor{blue}{cite}:
% \edit{
% \begin{equation}
%     P(x)= |\frac{1}{D}\sum_{i=1}^{n_g}e^{\frac{-j4\pi~D}{\lambda}}|^2 = n_g^2\bar{h}^2
% \end{equation}}
% %====MOcap_vs_Camera_AOA_accuracy interelement spacing====
% \begin{figure*}
% 	\centering
% 	\begin{minipage}{.45\linewidth}
% 	\centering
%     \includegraphics[width=7.5cm,height=6.0cm]{Images/AOA_mocap_allOnboard_data59EXP_sample_9.png}\\
%     \footnotesize\emph{{(a) Using Motion Capture Trajectory}}
% 	\end{minipage}
% 	\hspace{20pt}
% 	\begin{minipage}{.45\linewidth}
% 	\centering
%     \includegraphics[width=7.5cm,height=6.0cm]{Images/AOA_camera_allOnboard_data59EXP_sample_9.png}\\
%     \footnotesize\emph{{(b) Using Camera Trajectory}}
% 	\end{minipage}
% \caption{\footnotesize{\emph{Shows AOA profiles and Angle-of-Arrival for trajectories obtained in hardware experiments. Profile for oracle trajectory (left) with $0\%$ poorly-spaced antenna elements has almost no anomalous peaks compared to profile obtained using on-board sensor trajectory (right) with $15.74\%$ poorly-spaced antenna elements. Groundtruth AOA is $\phi=\ang{0}$ and $\theta=\ang{91}$. Note that the high AOA error for camera trajectory is a result of the combined effect of all the impact factors account of trajectory estimation error.}}}
% \label{fig:hW_results_inter-element_distance_AOA_mocap_vs_camera}
% \end{figure*}
% %====MOcap_vs_Camera_AOA_accuracy interelement spacing====
% We make the simplifying assumption of \edit{far-field line-of-sight in this expression. This is because the impact of antenna spacing might get marred by signal multipaths}. We fix $\bar{h}^2$, the power of the channel, to be fixed at each antenna in our array. We note that in practice, due to non-idealities and noise, $P(x)$ might be further attenuated, but for the purposes of this proof we assume that the well-spaced antennas and the poorly-space antennas are equally impacted by noise.

% The $n_b$ poorly-space elements contribute a peak at P($y$) of $n_b^2\bar{h}^2$. Thus, our final expression is:

% \begin{equation}
%     \frac{P(x)}{P(y)} \geq \frac{n_g^2}{n_b^2}
% \end{equation}
% We can thus infer that if the number of poorly-spaced elements is greater than well-spaced elements, the power of anomalous peaks would dominate thus giving a AOA value which is incorrect. Fig.~\ref{fig:Bad_element_percent_allOnBoard} shows the distribution for percentage of inter-element threshold violations for camera trajectories. Analysis of the wireless signal profile for one such hardware trial that compares motion capture and tracking camera trajectories is shown in Fig.~\ref{fig:hW_results_inter-element_distance_AOA_mocap_vs_camera}. The AOA profile with higher percentage of such violations (more poorly-spaced elements in camera trajectory) is much more noisier, leading to incorrect AOA estimation.

% \medskip
% \noindent Next we look at a special case of an ideal 2D circular trajectory and provide results from numerical analysis. \edit{Following the developments in~\cite{circularAntennaArrays} (Section 3.2.2) the referenced paper studies the phase mode excitation of a circular ring aperture - and in particular studies the effect of discretization (by using a finite element antenna array). This paper discusses the excitation of a array with phase mode $m$, $|m|\leq M$ where the resulting pattern
% \begin{align}
%     f_m^s(\mathbf{\theta})=\frac{1}{M}\sum_{n=0}^{N-1}e^{jm\gamma_n}e^{j\zeta\cos(\phi-\gamma_n)}
% \end{align}
% that can be expressed in terms of a combination of Bessel functions as
% \begin{align}
% \label{eq:main_term_sub_term_circularArray}
%     f_m^s(\mathbf{\theta})=j^mJ_m(\zeta)e^{jm\phi}+\sum_{q=1}^\infty (j^gJ_g(\zeta)e^{-jg\phi}+j^hJ_h(\zeta)e^{jh\phi})
% \end{align}
% This treatment seems to allow the separation of the \emph{desired response} $j^mJ_m(\zeta)e^{jm\phi}$ from the \emph{residual response} $\sum_{q=1}^\infty (j^gJ_g(\zeta)e^{-jg\phi}+j^hJ_h(\zeta)e^{jh\phi})$ which seems to capture the contribution of the anomalous terms resulting from discretization (using a finite number of antenna elements $N$). If $M$ is the order of the highest mode excited, the condition for the desired response to dominate is $N>2M$ which leads to the familiar requirement that inter-element spacing be kept below half a wavelength, i.e. $d<\lambda/2$.}



==> text/intro_v9.tex <==
\section{Introduction} \label{sec:intro}
Multi-robot coordination often requires robots to gather information about neighboring robots and their shared environment in order to collaborate effectively. Sensing relative state between robots, such as their relative positions, proximity, or nature (friend or foe) is often needed for coordination. This information is critical for various multi-robot applications, ranging from coverage, to exploration, to rendezvous and beyond ~\citep{bulloCoverage, almadhoun2019survey, cunningham2012fully, Freda20193DMP, Choudhary2016MultiRO, graphslam}. However, how to obtain this information in an unknown and unmapped environment, without line-of-sight
% (e.g. robots operating in different rooms), 
and without GPS or other external infrastructure, is an open challenge. A promising approach for obtaining relative position related information locally, exploits information extracted from exchanged wireless signals \citep{Gil2015AdaptiveCI}. As a wireless signal travels between robots, it physically interacts with the environment. Its amplitude and phase is affected by the distance it travels, the obstacles it passes through or is reflected off of, and the relative positions and velocities of the communicating robots in a phenomenon called \emph{multipath}. This multipath can be measured as an Angle-of-Arrival (AOA) profile, where the arriving signal's \emph{direction and power along each path} is measured as peaks along different spatial angles (see Fig.~\ref{fig:AOA_Profile}), for a pair of communicating robots in a team. Measuring these AOA profiles would thus allow robots to obtain information about the relative direction of other robots that they are able to receive any communication from, including lightweight ping packets. \emph{We note that ping packets incur a very small fraction of available bandwidth, as little as 5 KB/s; thus robots can perform AOA estimation of one another at much longer distances, and through occlusions, even if they are not able to communicate other information, such as maps, typically requiring much higher bandwidths~\citep{Schmuck2019CCMSLAMRA}.} In this way, wireless signals could inform about a distant or occluded neighboring robot which would be difficult or impossible to obtain using traditional on-board sensors alone such as LiDAR or camera.
%====AOA Profile Idea====
\begin{figure}
  \includegraphics[width=8cm,height=5.5cm]{Images/AOA_Profile.png}\caption{\footnotesize{\emph{Schematic representation of AOA profiles obtained by a signal receiving UAV for transmitting aerial and ground robot. Green, Red and orange lines represent the line-of-sight, direct and reflected signal paths respectively. These multipaths are captured in the corresponding AOA profiles as different AOA peaks.}}}
  \label{fig:AOA_Profile}
\end{figure}
%====AOA Profile Idea====

Previous work has shown that measuring AOA profiles is possible, and that incorporating this information into multi-robot systems can be used address several important long-standing challenges in robotics. For example: i) several AOA profiles collected from the same transmitting source can be used to triangulate the position of the sender, leading to accurate positioning and tracking in GPS-denied environments~\citep{ubicarse,spotFi,Xiong2013ArrayTrackAF,fadel3dTracking,Vasisht2016DecimeterLevelLW, fadelSeeThroughWalls,Karanam20173DTI}, ii) an AOA profile can be used by robots to find several directions of motion that would improve communication quality to another agent in the team, allowing for more reliable communication in complex and cluttered environments~\citep{Gil2015AdaptiveCI,Wang2019ActiveRF}, and iii) capturing the full multipath \emph{signature} of the sender via its AOA profile can be used to verify the uniqueness of a sender with implications for security and authentication in multi-agent systems~\citep{Gil2015Spoof-Resilient,securearray}. However, a main limitation of many of these approaches is that they do not extend to general robotics platforms and full 3D mobility of multiple agents, while maintaining the ability to collect AOA profile information. \emph{In order to achieve true adoption of this novel mode of sensing over communication signals in robotics, we need to resolve these important limitations which is the goal of the current paper.} In this paper we do not focus on a particular application domain but rather focus on the development of their critical primitive -- AOA profile measurement capabilities and the characterization of their attainable accuracy -- for general air/ground multi-robot systems.

We develop an algorithmic and theoretical framework for measuring full AOA profiles between robots that are i) communicating locally over a peer-to-peer standard WiFi network, ii) using only on-board sensors native to robotic platforms, namely, WiFi and a trajectory estimation sensor, and iii) freely mobile in 3D space. This framework would constitute a highly amenable design for fully distributed robotic systems. The key intuition for our approach builds off of Synthetic Aperture Radar (SAR) to measure small phase and amplitude differences of a transmitted WiFi signal as the receiving robot moves through space.  In this way, the robot effectively emulates \emph{``antenna arrays in the air},'' (See Fig. \ref{fig:Paper_schematic}) tracing out a virtual multi-antenna array (with one ``antenna element'' for each received packet) whose shape or \emph{array geometry} is dictated by the \emph{path traversed} by the robot. Antenna array theory indicates that a full AOA profile can be reconstructed from an array of short length of the order of signal wavelength (about 6cm for 5GHz WiFi) ~\citep{orfanidis2016electromagnetic}. This allows the receiving robot to resolve the incoming signal directions, using small displacements (sub-trajectories), as it moves through space. \textbf{This paper shows for the first time that arbitrary trajectories on general air/ground robotic platforms are indeed compatible with SAR-type approaches}.

Advances in accurate pose estimation of local robot trajectories using on-board sensors such as camera and LiDAR~\citep{Schmuck2019CCMSLAMRA, Choudhary2017DistributedMW,Qin2018VINSMonoAR} enable this new possibility of applying SAR over \emph{arbitrary} 2D and 3D trajectories on robot platforms. However, key challenges must be addressed. Namely, whether SAR-type approaches can be successfully employed over i) arbitrary 3D trajectories subject to trajectory estimation error, and ii) in a scenario where both the transmitting and receiving robot are moving simultaneously, was not known.

\subsection{Key challenges and approach}
We simultaneously address the challenges and opportunities imposed by arbitrary robot motion by appealing to antenna array theory~\citep{Vu2013-3D}. We first formulate a SAR equation to effectively isolate the phase change in the signal resulting from any arbitrary 2D or 3D robot trajectory. Isolation here refers to isolation of the phase change from other sources of noise, such as carrier frequency offset (CFO), and/or simultaneous mobility at the transmitting and receiving robots i.e \emph{\textbf{moving ends}}. Thus our developed methods allow for continuous data collection and AOA profile estimation, between any robots that can communicate (even at low rates of 5kB/s). 

Interestingly, the ability to perform SAR over arbitrary 3D robot trajectories holds potential for \emph{improving the accuracy of AOA profiles}. Thus, one key question that we address in this work is: \textbf{\emph{how to relate the informativeness of a robot's trajectory to the resulting AOA profile?}} It is well known that different antenna array geometries display different sensitivity to measuring phase differences in a received signal \citep{manikas2004differential}. 
% Since a robot traces out arbitrary virtual antenna array geometries by controlling its trajectory while sampling the received signal, 
% Specifically, it is intuitive to expect that different robot trajectories should also impact the sensitivity and resulting accuracy of the estimated AOA directions of a received signal. 
Hence, it is intuitive to expect that \emph{different robot trajectories should also impact the AOA profile and specifically the accuracy of the AOA peak that corresponds to the direction of maximum power path of received signal}. We formalize this intuition via a Cramer Rao Bound analysis. The Cramer Rao Bound (CRB) captures the sensitivity of AOA peak estimation, as it is a lower bound on its variance, resulting from a particular array geometry. In particular, the CRB is proportional to the inverse of the \emph{Fisher Information} for a specific antenna array geometry. We thus treat the inverse of the CRB as the \emph{informativeness} of the antenna array and seek to characterize this value for different trajectories. Along these lines we derive a new form of the CRB for analyzing the effect of arbitrary trajectory geometry on the quality of the resulting AOA estimation. Our analysis reveals that indeed the ability to compute AOA profiles over a robot's arbitrary 3D trajectories provides a precise advantage as 3D trajectories are highly informative when compared to 2D trajectories. 

% Our work shows that complex arbitrary robot trajectories can be broken down into simpler 2-D or 3-D geometries that permit this critical analysis. We then present a  re-formulated CRB analysis that provides useful insights for the error in angle-of-arriva for a larger class of irregular trajectories. 
Additionally, we derive the necessary theory to analyze the impact of the robot's trajectory estimation error, resulting from the use of on-board sensors, on the AOA estimation accuracy. Our theoretical development shows that trajectory drift and high frequency noise about the estimated trajectory mean manifests itself as a shift and attenuation of maximum magnitude AOA peak in the resulting profile, which we characterize. Moreover, we show that using short sub-trajectories makes our system resilient to long-term drift accumulation in the entire estimated robot trajectory. 
%====Paper idea Schematic====
\begin{figure}
  \includegraphics[width=8.7cm,height=5.0cm]{Images/Paper_idea_schematic.png}\caption{\footnotesize{\emph{A schematic representation of our approach that enables robots to sense relative direction of other robots using local trajectory and wireless signal information to emulate a virtual antenna array. The dotted black lines indicate arbitrary robot trajectory paths in 2D and 3D.}}}
  \label{fig:Paper_schematic}
\end{figure}
%====Paper idea Schematic====

\medskip
\noindent Our analysis reveals several surprising insights about the nature of how such robot trajectories influence AOA profiles, some of which are described below:
\begin{itemize}
\item \textbf{\ul{AOA profile reconstruction using arbitrary robot motion:}}. A single short local trajectory can be used to simultaneously measure AOA profiles for \emph{all} communication neighbor robots $j$ for a given robot $i$.
% \item \textbf{\ul{AOA profile reconstruction using arbitrary robot motion:}} Moving a robot $i$ by two wavelengths of motion (12cm for 5GHz WiFi) over arbitrary 2D or 3D paths can be used to reconstruct a full wireless signal AOA directional profile that can be used for sensing relative direction between any two communicating robots (c.f. Section~\ref{sec:Development}). One such local trajectory can be used to measure AOA profiles for \emph{all} communication neighbors $j$ of $i$ simultaneously.
\item \textbf{\ul{Informativeness of robot trajectories:}} A random curved trajectory in 3-D space of a given length is more informative (as determined by the CRB) than a regular linear trajectory, as might typically be prescribed for SAR. Hardware experiments support this analysis showing less than 10 $\deg$ error in AOA for 95\% of trials for arbitrary 3D trajectories, whereas for planar 2D curved and linear trajectories only 50\% and 7\% of trials show error below 10 $\deg$ respectively (c.f. Section~\ref{sec:cr-bound}).
\item \textbf{\ul{Influence of trajectory estimation error on AOA estimation accuracy:}} AOA estimation will suffer a shift $\Delta$ and a peak attenuation of $\cos(\sigma/2)$ where $\Delta$ is linearly proportional to the trajectory drift and $\sigma$ is the maximum angular variation of the trajectory estimation error about its mean (c.f. Lemma~\ref{lemma:trajError}). Our hardware experiments indicate that this translates to an estimation error of $10.03$ degree in azimuth, $2.23$ degree in elevation (use Fig. \ref{fig:AOA_SAR} schematic for reference) on average for $6\%$ absolute trajectory error (0.06m trajectory estimation error for a 1.2m robot displacement) using an Intel RealSense T265 off-the-shelf tracking camera. 
% \item \textbf{\ul{AOA estimation with moving ends:}} Obtaining AOA estimation using a SAR-based technique is possible even when both the transmitting and receiving robots are mobile during the signal sampling phase. We show that this is due to the translation agnostic property of AOA and can be accomplished under certain conditions (that we define) so long as robots can share their position estimates in their own local reference frame (c.f. Lemma~\ref{lemma:movingEnds}).
\item \textbf{\ul{AOA profile estimation with moving ends:}} Obtaining AOA estimation using a SAR-based technique is possible even when both the transmitting and receiving robots are mobile during the signal sampling phase. We show that this is due to the translation agnostic property of phase change in wireless signals. AOA estimation can thus be accomplished under certain conditions (that we define) so long as robots can share their position estimates in their own local reference frame (c.f. Lemma~\ref{lemma:movingEnds}). 
\end{itemize}  

%Moreover such \emph {relative trajectories} are naturally more informative since they introduce higher irregularity in the virtual antenna array geometry due to variation in transmitting and receiving robots speed and directions.

\noindent We substantiate the above observations with quantitative theoretical bounds on errors. These are further validated with extensive hardware experiments, demonstrating agreement in theory and in practice for every derived claim in the paper. Our implementation uses an off-the-shelf 5Ghz WiFi card, tracking camera, and a local-peer-to-peer network with no pre-installed wireless routers -- thereby demonstrating how our methods are designed for distributed implementation and seamless integration on today's robot platforms.
%Lastly, all of our theoretical and algorithmic developments are extensively tested in hardware, demonstrating agreement between theory and practice.  Further, our hardware experiments demonstrate the ability of our method to fuse data from on-board sensors like a VIO camera and received signal packets from off-the-shelf WiFi card, to calculate AOA. \textcolor{red}{It is to be noticed that our system doesn't require barebone network since all wireless packets would be requested and broadcasted in a peer-to-peer manner. Though we set our wireless protocol speed at lowest bitrate(6Mbps) of 5GHz WiFi, our system only requires 5kB/s bandwidth for wireless sensing and pose data. Combining that nature of our algorithm and local VIO, the system would work in a distributed way.} Thus, we demonstrate how our system is designed for seamless integration and continuous operation on today's robot platforms. 

%We implement and evaluate our system on  ground/aerial robots to sense all neighboring robots' signal direction using arbitrary 3D local trajectory. \textcolor{red}{Robots moving at 0.5 m/s max speed use their local ($\leq 1.5m$) sub-trajectory estimates and transmitted WiFi signals to infer} relative spatial distribution of other mobile agents, the AOA estimation is impacted only by error in local sub-trajectories obtained during the few seconds of data collection and not the drift in overall trajectory estimation. \textcolor{red}{For 0.04 ATE error in trajectory estimation we see an error of 5 degrees in AoA estimation.} Further, our hardware experiments demonstrate the ability of our method to fuse data from on-board sensors like a VIO camera and received signal packets from off-the-shelf WiFi card, to calculate AOA. \textcolor{red}{It is to be noticed that our system doesn't require barebone network since all wireless packets would be requested and broadcasted in a peer-to-peer manner. Though we set our wireless protocol speed at lowest bitrate(6Mbps) of 5GHz WiFi, our system only requires 5kB/s bandwidth for wireless sensing and pose data. Combining that nature of our algorithm and local VIO, the system would work in a distributed way.} Thus, we demonstrate how our system is designed for seamless integration and continuous operation on today's robot platforms. 

\subsection{Paper contributions} In this paper we:
\begin{enumerate}
    \item Develop the algorithmic machinery for using estimated local robot 3D trajectories for achieving incoming signal direction, or AOA profile estimation (Fig. \ref{fig:AOA_SAR}).
    \item Derive the algorithmic framework for allowing simultaneous motion of both ends (transmitting and receiving robots) while obtaining a full and accurate AOA profile. This accommodates continuous motion and continuous AOA estimation during robot operation.
    \item Develop the theory to characterize the impact of i) the robots' trajectory on the informativeness and accuracy of the AOA estimation and ii) trajectory estimation error on the AOA estimation error.
    \item Support all theory and algorithmic claims with in-depth hardware experiments, including a proof-of-concept application where robots use locally measured AOA to achieve fully dynamic rendezvous between an aerial drone and an occluded ground robot.
\end{enumerate}

\subsection{Paper roadmap} In the next section we provide a summary of previous work done in the context of robotics and wireless signal. Sec.~\ref{sec:Problem Formulation} formally states the problem statements and the definitions relevant to our development and analysis. Sec.~\ref{sec:Development} details the formulation of arbitrary 3D SAR and  Sec.~\ref{sec:moving_ends} shows how our system can handle signal transmitter robots that are mobile. Sec.~\ref{sec:Analysis_impact_factors} provides an analysis of the different factors that impact AOA calculation. We show the results of our hardware experiments in Sec.~\ref{sec:results} and evaluate the capability of our system using a proof-of-concept application in Sec.~\ref{sec:hardware_application}. Finally, we provide directions for future research and concluding remarks in Sec.~\ref{sec:discussion} and~\ref{sec:conclusion} respectively.
%====AOA SAR Schematic====
\begin{figure}
  \includegraphics[width=8.7cm,height=7.0cm]{Images/AOA_SAR_Schematic_3.png}\caption{\footnotesize{\emph{Schematic showing AOA profile obtained by signal receiving UAV for transmitting ground and aerial robots. The Angle-of-Arrival ($\phi,\theta$) in azimuth (top view) and elevation (side view) respectively obtained from these profiles is highlighted in yellow.}}}
  \label{fig:AOA_SAR}
\end{figure}
%====AOA SAR Schematic====

==> text/moving_ends.tex <==
\section{Moving Ends Formulation}\label{sec:moving_ends}
%=========Formulation 1 - for MOCAP =========
%In the previous section we show that how a robot can calculate AOA to other robots using the wireless channel information. 
% \textcolor{red}{\textbf{NEED REVIEW} In this section we show how our approach can be used even when two robots are moving simultaneously. Essentially we show that a moving robot 'i' can calculate AOA to another moving robot 'j' by using relative trajectory obtained from it's own and robot 'j' local trajectory, given that both robots have the same heading. Given trajectories in euclidean coordinates $\text{X}_i$ = \{$p_i(t_k)$, $p_i(t_{k+1})$,... $p_i(t_l)$\} and $\text{X}_j$ = \{$p_j(t_k)$, $p_j(t_{k+1})$,... $p_j(t_l)$\} of two moving robots $i$ and $j$ in a global coordinate frame of reference, (see Fig.~\ref{fig:Moving_ends_schematic}), the relative trajectory of robot $i$ for timesteps $t_k$ to $t_l$ is given by $\text{X}^r_i$ = $\text{X}_i$ - $\xt{X}_j$ , where \forall ~$p^r_i(t)$\in $\text{X}^r_i$,  $p^r_i(t)$ = ($p_i(t)$ - ($p_j(t)$), i.e 
% \begin{equation}\label{eq:rho_1}
%       p^r_i(t_k) =  (p_i(t_k) - (p_j(t_k)) - ((p_i(t_1) - (p_j(t_1)))
% \end{equation}
% \noindent Now, given normalized trajectory in a global frame of reference, we can derive a similar equation for $x^r_i(t_k)$. Let the normalized  trajectories be $\text{X}_i$ = \{0, $x_i(t_2)-x_i(t_1)$,... $x_i(t_k)-x_i(t_1)$\} and $\text{X}_j$ = \{0, $x_j(t_2)-x_j(t_1)$,... $x_j(t_k)-x_j(t_1)$\} of two moving robots in a global coordinate frame of reference, (see Fig.~\ref{fig:Moving_ends_schematic}), the relative trajectory of robot $i$ is given by $\text{X}^r_i$ = $\text{X}_i$ - $\text{X}_j$ , where \forall ~$x^r_i(t_k)$\in $\text{X}^r_i$,  $x^r_i(t_k)$ = ($x_i(t_k)$ - $x_i(t_1))$ - ($x_j_(t_k)$ - $x_j_(t_k)$). Rearranging the terms we get:
% %Thus we can obtain $\rho$ as 
% % \begin{align*}
% %       \rho^r_i(t_k) =  ((x_i(t_k)- (x_i(t_1)) - ((x_j(t_k) - (x_j(t_1))) - 0)
% % \end{align*}
% \begin{equation}\label{eq:rho_2}
%       x^r_i(t_k) =  (x_i(t_k) - (x_j(t_k)) - ((x_i(t_1) - (x_j(t_1)))
% \end{equation}}
% \noindent Thus from Equation~\eqref{eq:rho_1} and ~\eqref{eq:rho_2}, we see that two normalized trajectories in a same frame of reference can be used to calculate a relative trajectory between them. But in reality we do not have access to such global frame of reference and the local frames of the robots have a rotation and translation offset. We introduce the following lemma which shows how a robot can achieve accurate AOA in the presence of these offsets. We assume that the robots know the true \emph{North} and true \emph{Down} direction using onboard sensor like magnetometer and gyroscope/gravity sensor respectively. 

In this section we generalize our framework from Sec.~\ref{sec:Development} to accommodate the case where both receiving and transmitting robots are moving simultaneously during the data collection phase. This case is particularly challenging since not accounting for relative displacements between agents can greatly impact the resulting signal phase measurements -- leading to errors in the generated AOA profile $F_{ij}(\phi,\theta)$. Here, we show that a receiving robot $i$ can calculate $F_{ij}(\phi,\theta)$ to a moving transmitting robot $j$ by using the relative trajectory obtained from it's own and robot $j$'s local trajectory estimates -- namely, by using $\boldmath{\chi_{ij}}\textbf{(t)}$ as the steering vector (Fig. \ref{fig:Moving_ends_schematic}). One clear difficulty in computing $\boldmath{\chi_{ij}}\textbf{(t)}$ is that robot $i$ and robot $j$ \emph{do not share a common coordinate reference frame} in the most general case. However, we begin the development of this section assuming the availability of a shared reference frame and then generalize to the case of different local coordinate frames between agents.

For the time being, let us assume that the robots have a common frame of reference (an assumption that we later relax). Thus, any position $p_{ij}(t)$ for pose $\chi_{ij}(t)$ in robot $i$'s relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ for $t \in [t_k,\hdots,t_l]$ is given as:
\begin{equation}\label{eq:rho_1}
      p_{ij}(t) =  (p_i(t) - p_j(t)) - (p_i(t_k) - p_j(t_k))
\end{equation}
This is because all poses in the local trajectory $\boldmath{\chi}_i\textbf{(t)}$ are relative to the starting pose $\chi_i(t_k)$ in the trajectory for any robot $i$. Essentially, as our method uses the `local sub-trajectory' with respect to the pose at time $t_k$ for any given robot, the relative poses obtained as per Eqn.~\eqref{eq:rho_1} can thus be applied to obtain steering vector. $F_{ij}(\phi,\theta)$ can then be calculated with the same 3D SAR formulation developed in Sec.~\ref{sec:Development}.

In reality however, we do not have access to a global frame of reference and the local coordinate frames of the robots will have a rotation and translation drifting offset compared to global frame, thus making the computation of a relative trajectory difficult to obtain. We introduce the following lemma which shows how a robot can obtain $F_{ij}(\phi,\theta)$ in the presence of these offsets. We first define the concept of a \emph{null vector} which captures the translation independent character of wireless signal phase measurements.

\begin{definition}[\underline{Null Vector}]:   We define the \emph{Null Vector} of a receiving robot $i$ as a vector along a specific angle-of-arrival from it's start position $p_i(t_k)$. A transmitting robot $j$ at any position on this \emph{Null Vector} and performing the same trajectory motion will lead to same change in \emph{phase} of the wireless signal intercepted by robot $i$ (see Fig. \ref{fig:null_vector}).
\label{def:Null_vector}
\end{definition}

\noindent This is due to the fact that channel phase measurements are independent of the distance between a signal transmitter and receiver (for a detailed discussion, refer \citep{Ioannides2005UniformCA}). Thus, using the concept of a \emph{Null vector} we show that robots sharing a common North vector and gravity vector is sufficient to compute $\boldmath{\chi_{ij}}\textbf{(t)}$ as needed by our steering vector in Eqn.~\eqref{eqn:steering_vector}.
%====Null vector and Moving End schematic=======
\begin{figure}
	\centering
	\includegraphics[width=8.0cm,height=6.5cm]{Images/Null_Vector.PNG}
	\caption{\footnotesize{\emph{Schematic representation of the Null vector of robot $i$ (performing 3D SAR) for Angle-of-Arrival ($\phi$,$\theta$). Rotation offset between any robot $j\in\mathcal{N}_i$ and robot $i$'s local coordinate frames can be removed by aligning the robots to true NORTH and DOWN direction (using on-board sensors like magnetometer and gyroscope/gravity sensor). At any position on Null vector (e.g position A and B), robot $j$ will lead to same phase change in WiFi signal, if the trajectory geometry is same (dotted red line).}}}
	\label{fig:null_vector}
\end{figure}
%====Null vector and Moving End schematic=======

\begin{lemma}
\label{lemma:movingEnds}
Given trajectories of two robots $i$ and $j\in\mathcal{N}_i$, each in their own local frame of reference with rotation offset $\tilde{R_i}$, $\tilde{R_j}$ with respect to a shared North vector, and a shared gravity vector and translation offset $\tilde{t}_{ij}$ with respect to each other, robot $i$ can calculate relative $AOA_{max}$ to robot $j$ by correcting for rotation offset and ignoring the translation offset.
\end{lemma}

\noindent \textit{Proof: } As stated in our assumptions in Sec.~\ref{sec:Problem Formulation}, on-board sensors like magnetometer and gyroscope/gravity sensor can be used to rotate $\boldmath{\chi_i}\textbf{(t)}$ of a robot $i$ towards true \emph{North} and \emph{Down} by applying a rotation matrix, i.e $\boldmath{\tilde{\chi_i}\textbf{(t)}}$ = $\tilde{R_i}\hspace{-4pt}$ $\boldmath{\chi_i}\textbf{(t)}$. Similarly any robot $j\in\mathcal{N}_i$ can align its coordinate frame such that $\boldmath{\tilde{\chi_j}\textbf{(t)}}$ =  $\tilde{R_j}\hspace{-4pt}$ $\boldmath{\chi_j}\textbf{(t)}$. Following Defn.~(\ref{def:Null_vector}), a robot $j$ at a true AOA of angle of ($\phi$,$\theta$) to robot $i$ will give similar \emph{AOA} using our approach as long as it's anywhere on the \emph{Null Vector} and performing same motion (Fig. \ref{fig:null_vector}). The relative trajectory can thus be obtained as $\boldmath{\chi_{ij}\textbf{(t)}}$ = $\boldmath{\tilde{\chi_i}\textbf{(t)}}$ - $\boldmath{\tilde{\chi_j}\textbf{(t)}}$, since the presence of a translation offset $\tilde{t}_{ij}$ does not impact $AOA_{max}$ calculation and one can use Eqn.~(\ref{eq:rho_1}) to compute the steering vector. We validate our approach in hardware experiment  (Fig. \ref{fig:Relative_Traj_comparison_3D}), demonstrating our ability to compute $F_ij(\phi,\theta)$ for this moving ends problem in the Results Section of this paper (Sec.~\ref{sec:results}). As stated in our assumptions, the relative AOA is always computed with respect to position $p_i(t_k)$ of receiving robot $i$. Therefore we assume that robots are far enough away from each other such that local motions (which could be as small as 12cm when WiFi is used) will not significantly change their true relative AOA.
% \footnote{In practice we find that a separation of 2 m is sufficient for robots traveling at 0.6m/s relative velocity.}.

\medskip
%In fact given that both the signal transmitter and receiver robots would be moving along different directions and at different speeds, we can expect to obtain a trajectory shape that has more information. 
In the next section we analyze the impact of different trajectory shapes on $F_{ij}(\phi,\theta)$, i.e. we characterize trajectory \emph{informativeness}. We also characterize the effect of errors in trajectory estimation on \emph{AOA}.  


==> text/problem.tex <==
\vspace{-5pt}
\section{Problem Formulation}\label{sec:Problem Formulation}
This paper aims to enable robots in a team to infer relative spatial directions, i.e an Angle-of-Arrival (AOA) profile $F_{ij}(\phi,\theta)$ to others in its neighborhood, based on received communication signals between them. In doing so, we aim to develop an ``inter-robot sensor'' for robots to obtain relative directional information about each other by analyzing existing \emph{communication packets} in the network. We leverage off-the-shelf WiFi modules for this purpose. Specifically, our goal is to find ${F_{ij}(\phi,\theta)}$. Of particular interest is finding the maximum magnitude path $AOA_{max}$, between the robots referred to as the \emph{azimuth angle $\phi$} and \emph{elevation angle $\theta$} to a neighboring transmitting robot (see Fig.~\ref{fig:3DcoordinateSystem})\footnote{We note that in some cases the strongest signal path may not be the direct path which might be attenuated due to absorption or reflection of signals. However in this case there exist many methods for inferring the direct path ~\citep{ubicarse,spotFi}. In this paper we do not address the problem of finding the direct path from $F_{ij}(\phi,\theta)$ and rather refer the reader to relevant references for the solution to this problem.}. Our system uses an approach akin to Synthetic Aperture Radar for this purpose. Key challenges for applying SAR-based methods to heterogeneous robot systems that we aim to address in this paper are: 
\vspace{-3pt}
\begin{enumerate}
    \item \textbf{Mobility:} Developing a framework to support AOA profile generation where both the transmitting and receiving robots are simultaneously mobile along arbitrary 2D or 3D trajectories during data capture. This is a commonly encountered scenario in multi-robot teams that must be accounted for in our SAR formulation in order to allow for continuous AOA sensing capabilities amongst the robots.
    \item \textbf{Trajectory geometry:} Characterizing \emph{informativeness}, or the impact of \emph{robot trajectories} on the sensitivity of the resulting phase measurements and the resulting $F_{ij}(\phi,\theta)$. We do so by studying the impact of \emph{antenna array geometry} on the accuracy of the $AOA_{max}$ which is not readily known for arbitrary shapes such as those generated by arbitrary robot trajectories. 
    \item \textbf{Estimation Noise:} Analyzing the effect of trajectory estimation error on $F_{ij}(\phi,\theta)$. In real robotic systems it is possible to obtain local robot displacement estimates using various tools such as inertial measurements and VIO, however it is well known that these estimates are subject to noise.  Thus the impact of this estimation noise on the accuracy of the resulting $AOA_{max}$ estimation must be quantified.
\end{enumerate}
\subsection{Simultaneous robot motion}
As many previous approaches that use SAR to obtain $AOA_{max}$ require transmitting robots to remain static during the period of data collection~\citep{Wang2019ActiveRF,PinIt,mostofiAOA}, they are not feasible for applications that require continuous mobility of all the robots. Additionally, they do not account for arbitrary motion of robots in 2D and 3D. This necessitates that our system account for motion of both signal transmitting and receiving robots and we refer to this as the \emph{moving ends} problem. 
\begin{problem}[Moving ends problem] 
Given WiFi signal receiving robot $i$'s local trajectory from position $p_i(t_k))$ to $p_i(t_l))$ and transmitting robot $j$'s,  $j\in\mathcal{N}_i$, local trajectory from position $p_j(t_k))$ to $p_j(t_l))$, obtain $F_{ij}(\theta,\phi)$ where $\textbf{a}(\phi,\theta)\textbf{(t)}$ characterizes robot $i$'s relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ with respect to robot $j$.
\end{problem}
\noindent We first formulate the SAR based solution in Sec. \ref{sec:Development} for obtaining $F_{ij}(\phi,\theta)$ from arbitrary 3D motion of receiving robot, by applying the concepts from antenna array theory (Fig. \ref{fig:3D_SAR_AOA}). In Sec. \ref{sec:moving_ends} we use this formulation of 3D SAR for a static transmitting robot to solve the moving ends problem. 

\subsection{Information gain from trajectory geometry}
Our formulation can leverage different robot trajectory shapes in 2D and 3D to emulate virtual antenna arrays of varying geometry. It is well known that an array's geometry affects its sensitivity to differentiate phases of an arriving signal from different source locations \citep{manikas2004differential}. For the case of interest in this paper where robots can operate in the full 3D space (not just 2.5D), sensitivity of the array and the ability to estimate $AOA_{max}$ consistently independent of source location, is of utmost importance. For the purposes of characterizing the sensitivity of a particular antenna array geometry, the Cramer Rao Bound (CRB) is often employed~\citep{Gazzah2006CramerRaoBF}. The Cramer Rao Bound is a lower bound on the variance of the $AOA_{max}$ estimation resulting from a particular antenna array geometry and is given by (dropping $t$ and subscript $i$,$j$ for brevity):
\begin{align}
    &CRB = 
\begin{bmatrix}
C_{\theta \theta} & C_{\theta \phi} \\
C_{\phi \theta} & C_{\phi \phi} \\
\end{bmatrix} \nonumber \\
&=\frac{\sigma^2}{2\mathbf{h}^H\mathbf{h}}{\underbrace{\begin{bmatrix}
Re(\frac{\partial a^H(\theta,\phi)}{\partial\theta} \frac{\partial a(\theta,\phi)}{\partial\theta}) &  Re(\frac{\partial a^H(\theta,\phi)}{\partial\theta} \frac{\partial a(\theta,\phi)}{\partial\phi}) \\
Re(\frac{\partial a^H(\theta,\phi)}{\partial\phi} \frac{\partial a(\theta,\phi)}{\partial\theta}) & Re(\frac{\partial a^H(\theta,\phi)}{\partial\phi} \frac{\partial a(\theta,\phi)}{\partial\phi})
\end{bmatrix}}_{FIM}}^{-1}
\label{eq:CRB_equation}
\end{align}

\noindent for a particular source direction indicated by its azimuth angle $\theta$ and elevation angle $\phi$. Here $\sigma^2$ is the variance in noise of the wireless signal. FIM is the \emph{Fisher Information Matrix} which measures the amount of information that the geometry of the antenna array (captured via $\textbf{a}(\theta,\phi)\textbf{(t)}$ i.e the steering vector) provides on $F_{ij}(\phi,\theta)$. Since in our problem formulation the geometry of the virtual antenna array is dictated by the trajectory of the receiving robot, we define the \emph{informativeness} of a trajectory using the CRB as follows.

\begin{definition}[\underline{Informativeness}]:
We say that a trajectory is more \emph{informative} than another if it permits a smaller variance in $AOA_{max}$ as dictated by the Cramer Rao Bound (CRB).
\label{def:Informativeness}
\end{definition}

\noindent Thus, the second problem that we wish to tackle in this paper is the characterization of the informativeness for different robot trajectories; i.e. the effectiveness of our $AOA_{max}$ estimation capabilities as a function of the trajectory traversed by a robot as it is receiving communication packets from its neighbors.

\begin{problem}[Informativeness]
We wish to derive the formulation for the Cramer-Rao Bound (cf. Eqn.~\eqref{eq:CRB_equation}) in the $\theta$ and $\phi$ directions for arbitrary 3D robot trajectories, thereby characterizing the \emph{informativeness} of different robot trajectories.
\end{problem}

\noindent Sec. \ref{sec:cr-bound} details the theoretical development our CRB analysis for three types of common robot trajectories: 3D helix, 2D planar circular and 2D linear. Our experimental analysis further shows that the insights garnered for these trajectory types generalize to overall trends in arbitrary 2D and 3D robot trajectories. 

% We note that in the extreme case, some trajectory geometries such as linear or 2D planar arrays suffer from \emph{ambiguities}. 
% \begin{definition}[\underline{Ambiguity}]
% We say that an AOA profile is ambiguous, when two distinct signal source locations will result in the same measured phase differences at the receiving antenna.
% \label{def:ambiguity}
% \end{definition}
% \noindent For example, a linear antenna array will exhibit left/right ambiguity and a planar 2D antenna cannot not differentiate between a source in the plane above the array versus a source in the plane below the array. This is a well know problem in antenna array theory ~\citep{manikas2004differential} and in Sec. \ref{sec:results_informativeness} we show results that this is greatly alleviated by using trajectories with high informativeness.

\subsection{Impact of trajectory estimation error}\label{sec:ps_trajectory_impact}
Although our approach is independent of how such robot trajectories are obtained, in order to make our system native to robotic platforms, our goal is to leverage trajectory estimates from on-board sensors (e.g VIO camera). Therefore, the third problem that we address in this paper is to characterize, both analytically and experimentally, the impact of the receiving robot's trajectory estimation error on its generated $F_{ij}(\phi,\theta)$. In this paper, we use robot trajectories of the following two types to test our system's performance: 
\begin{itemize}
    \item \textit{\underline{Groundtruth trajectory}}: obtained using position estimates from motion capture system denoted by $p(t)$ at time $t$.
    \item \textit{\underline{Tracking camera trajectory}}: obtained using position estimates from Intel Realsense T265 tracking camera. This out-of-the-box camera runs a visual SLAM algorithm which provides pose estimates at 200 Hz. We denote the estimated position at time $t$ as $\hat{p}(t)$.
\end{itemize}

\noindent Using trajectories from tracking camera introduces error in $F_{ij}(\phi,\theta)$ on account of noisy trajectory estimation. A commonly used metric to quantify error in trajectory estimation is Absolute Trajectory Error~\citep{Sturm2012ABF,Choudhary2017DistributedMW}, given by the equation below
% \begin{definition}{\underline{$ATE_{trans}$}:}
\begin{equation}
    \label{eq:ATEtran}
    ATE_{\text{trans}} = \left(\frac{1}{n} \sum_{t=t_{k}}^{t_{l}} ||p(t) - \hat{p}(t) ||^2\right)^{\frac{1}{2}}
\end{equation}
% \end{definition}
% ,where $p(t)$ is the local position estimate of a robot and $\hat{p}(t)$ is the groundtruth position. 
As ours is a relative direction finding system that uses spherical coordinates, we use an angular drift metric \citep{angulardrifting} for our theoretical analysis to quantify the error in trajectory\footnote{For empirical evaluation, the corresponding $ATE_{trans}$ is calculated in Cartesian coordinates for simplicity.}. This is given as:
\begin{definition}[\underline{Angular drift}]:
For every groundtruth position in a robot trajectory $p(t) = (\rho,\varphi,\xi)$, we get an estimated position $\hat{p}(t)=((\rho-\kappa_{\rho},\varphi-\kappa_{\phi},\xi-\kappa_{\theta}))$, whenever $\kappa_{\phi}$, $\kappa_{\theta}$ are constant or varying angular error and $\kappa_{\rho}$, we say that the trajectory has an angular drift. 
\label{def:angular-drift}
\end{definition}

\noindent Since a robot's trajectory is used to generate the full $F_ij(\phi,\theta)$ (cf. Eqn.~\ref{eqn:bartlett_estimator}), an error in trajectory estimation will result in an error in $AOA_{max}$ calculation between two robots. We define this error to be \emph{AOA Estimation Error}.

\begin{definition}[\underline{AOA error}]:  We define error in AOA as $\phi_g - \hat{\phi}$ in azimuth and $\theta_g - \hat{\theta}$ in elevation, where ($\phi_g,\theta_g$) is the true AOA to the signal transmitting robot and ($\hat{\phi},\hat{\theta}$) is the estimated \emph{AOA} obtained by our system. 
\label{def:AoA-error}
\end{definition}
\noindent We use L2 norm between estimated $AOA_{max}$ and true AOA, as an error metric given by the equation:
\begin{equation}AOA_{Error} = \sqrt{(\phi_g - \hat{\phi})^{2} + (\theta_g-\hat{\theta})^{2}}
\label{eqn:AOA_euclidean_error}
\end{equation}

\noindent Thus we can now define our problem of characterizing the impact of trajectory estimation error on AOA error as:

\begin{problem}[Impact of trajectory estimation error]
For nonzero trajectory estimation error $ATE_{\text{trans}}$, we wish to characterize the effect of angular drift  $\kappa_{\phi}>0$, $\kappa_{\theta}>0$ on the error, $AOA_{Error}$ in Eqn.~\eqref{eqn:AOA_euclidean_error}, in our measured $AOA_{max}$. 
\end{problem}

\noindent We note that in practice AOA error can arise from simultaneous impact of many factors, including insufficient informativeness of robot trajectories, artifacts from AOA estimation algorithms or errors in robot position estimation, and channel noise or unaccounted for phase shifts due to \emph{Carrier Frequency Offset} (CFO) or mobility of robot platforms (i.e. the \emph{moving ends} problem). In this paper we analyze the effects of these sources of error on $F_ij(\phi,\theta)$ independently.

\medskip
Finally, we aim to extensively validate our system's accuracy and performance on real robotic platforms in 2D and 3D space. In Sec. \ref{sec:hardware_application}, we evaluate the utility of our system for a dynamic rendezvous experiment based different trajectory geometries generated during navigation in an unmapped environment in presence of moving ends and occlusions in the environment.

\medskip 
\noindent We summarize key assumptions used throughout the paper:
\begin{assumption*}[Common paper assumptions].
 
\begin{enumerate}
    %\item The transmitting and receiving robots are far enough so that the signal waves are planar (Eqn. \ref{eqn:channel_basic_eqn}). 
    \item Robots know the true \emph{North} and true \emph{Down} direction using on-board sensor like magnetometer and gyroscope/gravity sensor respectively.
    %\item Impact of $\kappa_{\rho}$ (error in $\rho$) is negligible for small trajectories compared $\kappa_{\phi}$, $\kappa_{\theta}$ and thus it does not impact AOA.
    \item Each robot has the same global clock to match forward-reverse channel packets based on timestamps used subsequently for canceling the effects of \emph{carrier frequency offset} (CFO). 
    \item All AOA measurements are taken with respect to the initial position $p_i(t_k)$ of robot $i$ in its local frame. 
\end{enumerate}
\end{assumption*}

\medskip
In the next section we derive our general formulation for 3D arbitrary trajectory SAR and demonstrate how a moving robot can use it for obtaining relative $AOA_{max}$ to a static transmitting robot. Following this, we show how our formulation can be extended to address the full mobility case, i.e. the moving ends problem. 




==> text/related-work.tex <==
\section{Related Work}\label{sec:related_works}
In this section, we provide an overview of prior work on applications of wireless signals, specifically in the context of robotics. We first highlight some of the limitations of traditional sensors in obtaining relative information in multi-robot systems, as well as developments in wireless community that explore the use of wireless signals as a sensing modality. Next we look at previous approaches on obtaining relative direction information between communicating robots, the corresponding open challenges and the underlying enabling research from antenna array theory and computer vision. 
%% SAR References (2D, 3D, Circular)


%% Frontier Exploration References


%% Coverage References


%% Optical Flow References


%% Cramer Rao Bound for Error Analysis 


%% SLAM and ORB-SLAM References

%%Include *structure from motion* references
% This section summarizes work done in three areas that relate to our proposed system - robotics wireless sensor networks, systems that use synthetic aperture radar or AOA information, and visual inertial odometry.
\subsubsection*{\textbf{Relative state estimation in multi-robot systems:}}
Many multi-robot coordination problems such as coverage~\citep{bulloCoverage}, mapping~\citep{robotMapping_fingerprints_Roland,mappingMonocularSLAM,featuresMapping,cooperativeMapping_leonard}, frontier exploration~\citep{Gautam2017FASTS, Solanas2004CoordinatedME, Fox2005DistributedME,multiagentExploration_BurgardThrun}, and persistent surveillance~\citep{persistentSurveillance_experiments,persistentSurveillance} rely on knowledge of relative positions and other state information between collaborating robots. This information can be obtained from on-board GPS devices or other sensors such as camera and LiDAR that provide information of other agents' relative poses as well as about the environment; a capability useful for many of the stated collaboration tasks, but they have important limitations. In particular they often don't work in GPS-denied and communication constrained environments, non-line-of-sight, over long distances, and/or when there is a lack of a shared coordinate frame and map. Thus, for many common environments such as those with clutter, those that require robots to operate at far distances from one another or the ones that lack common features required for fixing a shared coordinate frame, the current sensing methods easily get disoriented~\citep{SajadSaeedi2016MultipleRobotSL,multislamKshirsagar2018ASO}.
%===hardware robots=====
\begin{figure}
        \includegraphics[width=8.5cm,height=4.0cm]{Images/hardware_setup_robots.PNG}
    	\caption{\footnotesize{\emph{Aerial and ground robots used in hardware experiments equipped with different off-the-shelf on-board sensors. Each robot is equipped with an UP Squared on-board compute device that has Intel 5300 WiFi card, an omnidirectional antenna, and an Intel RealSense T265 tracking cameras.}}}
    	\label{fig:hardware_robots}
\end{figure}
%===hardware robots=====

\subsubsection*{\textbf{Sensing using wireless signals:}}
Going beyond traditional sensors, a robotic platform can we equipped with different types of wireless communication hardware \citep{CalvoFullana2019MultimodeAC}. Beyond enabling communication, wireless signals processing has shown great promise for sensing as well. For example, it has been shown that transmitted wireless signals between devices can be used to extract useful information such as device position~\citep{spotFi,Xiong2013ArrayTrackAF,lteye,PinIt,mostofiAOA,Cominelli2019DeadOA,Verma2018DOAEF}. Beyond localization, recent work has shown the ability to sense rich information about the environment as well, from tracking and imaging behind walls~\citep{fadelThroughWallSensing,mostofi_throughWall_wirelessSensing,fadelSeeThroughWalls,mostofi_wirelessSensing_mapping}, to materials sensing~\citep{swarun_materialSensing, fadel_foodSensing, Dhekne2018LiquIDAW}, imaging in harsh visual conditions \citep{Guan2020ThroughFH} and even shape sensing~\citep{swarun_shapeSensing}. While these works undoubtedly show the promise of using wireless signals to obtain useful information about a robots' state and its environment in ways that more traditional sensors like cameras and LiDAR cannot, they are not necessarily compatible with general robotics applications. These methods sometimes use specialized hardware, specialized wireless signals and non 802.11 protocols  (that may not be WiFi which are most readily available on robot platforms) or pre-deployed infrastructure. Often, they also do not consider mobility (both signal transmitting and receiving robot), which can have a profound impact on the accuracy of these methods. As such, they are not inherently designed to be seamlessly integrated with robotic platforms. 

Some WiFi based methods use Received Signal Strength (RSS), which refers to the magnitude of the signal \citep{Zhu2013RSSIbasedAF}. However capturing substantial changes in signal magnitude require large displacements of the receiving robot and/or requires sampling along multiple directions. This makes RSS coarse and hence ill-suited for extracting information with accuracy and precision over short robot displacements. Another possibility is to use \emph{Channel State Information} (CSI) - information obtained from the PHY layer of 802.11 protocol \citep{Halperin2010Predictable8P}. CSI essentially facilitates capturing the phase of a wireless signal which is very sensitive to even small amount of displacements. It thus provides more granularity of information as compared to RSS ~\citep{Yang2013FromRT,Ma2019WiFiSW}.
\subsubsection*{\textbf{Synthetic Aperture Radar (SAR):}}
Using mobility of robots can improve the quality of information obtained \citep{Twigg2019RoboticPA}. SAR is also an alternative solution to obtain information from wireless signals that leverages mobility of signal receivers \citep{sar1998}. Applications for imaging that use RADAR-based SAR, generally use controlled linear motion of robot arm or alternatively they mount a vertical linear array on the robot~\citep{Watts20162DA3,Barrie2004ThroughWallSA}. On the other hand, our previous work \emph{exploits mobility} and WiFi signals, both inherent to robotic platforms, to emulate a virtual antenna array along the trajectory of the robot, a method akin to SAR for accurately measuring the change in phase of an incoming signal. As WiFi signals traverse between a transmitting robot and a receiving robot, they interact with the environment such as being absorbed, reflected, and scattered \citep{Goldsmith2005WirelessC} by objects in the environment. Therefore, the signal paths a particular communicated message takes through the environment if properly resolved, can reveal information about the direction of the transmitting robot. This proves useful in absence of a global reference frame where the robots are separated by large distances and/or are occluded by objects in the environment. Indeed, exploiting this fact has led to many uses like positioning~\citep{ubicarse}, adaptive networking~\citep{Gil2015AdaptiveCI}, mapping~\citep{Wang2019ActiveRF}, and security~\citep{Gil2015Spoof-Resilient,icra2019,Gil2019ResilientMC}. These works use position information from simple linear motion or 2D circular trajectories (e.g. turn-in-place) obtained using IMU and require that the transmitting robot should be static over the data collection period of a few seconds.

% However, limited by typical formulation of antenna array, these works require prescribed robot motion along simple linear or 2D circular trajectories such as a turn-in-place. They also require that over the data collection period of a few seconds, the other robotic agent should be static~\citep{Wang2019ActiveRF}, \textcolor{green}{as even small displacement of the signal transmitter (equivalent to one wavelength or 6 cm for 5GHz channels), if not accounted for, leads to phase shift of 2*PI leading to considerable errors in phase measurements}. These requirements are unfortunately not always satisfiable by all robotic systems and also results in some sensing ambiguity since simple trajectories (like linear or planar circular) do not exploit the full range of motion and thus geometry, of antenna arrays that they are emulating. Indeed antenna array research shows that 3D antenna arrays are superior to 2D arrays in terms of accuracy and richness of information that can be extracted from received wireless signals~\citep{Vu2013-3D, Vu2010PerformanceAO}. Specifically, 2D antenna array would suffer from ambiguously symmetric geometry. These factors are important motivators for developing the ability for robots to \emph{emulate 3D antenna arrays over their arbitrary paths as they traverse the environment.}
However, emulating a linear or circular antenna array leads to \emph{sensing ambiguities} where the receiver robot in unable to distinguish between two (or more) transmitter robot directions. For example, a linear antenna array will exhibit left/right ambiguity and a planar 2D antenna cannot not differentiate between a source in the plane above the array versus a source in the plane below the array. This is a well know problem in antenna array theory~\citep[chapter 6]{manikas2004differential}. Antenna array research shows a possible solution of using 3D antenna arrays that are capable of resolving such ambiguities~\citep{Vu2013-3D, Vu2010PerformanceAO}, but this requires emulating an arbitrary shaped 3D array using position information from on-board sensors. Another open challenge not addressed by previous works is the possible mobility of the transmitting robot for the duration of SAR. The change in phase measurements for even small displacements (e.g 24cm) of the receiving robot is desirable for obtaining highly accurate AOA profile \citep{Gil2015AdaptiveCI}. However if the simultaneous motion of the transmitting robot on the same scale, if not accounted for, leads to phase shift of 2*$\pi$ resulting in considerable errors in phase measurements for the receiving robot. These factors are important motivators for developing the ability for robots to \emph{emulate 3D antenna arrays over their arbitrary paths as they traverse the environment while both ends (i.e transmitting and receiving robots) remain mobile at all times.}

\subsubsection*{\textbf{Trajectory estimation:}}
Advances in vision-based sensing and optimization in the past couple of years allow for obtaining accurate local trajectory estimates. Monocular systems such as \citep{Qin2018VINSMonoAR}, utilize one camera and one low-cost inertial measurement unit as sensing components, achieving 0.21m ATE in a 500m real world trajectory. Pose Graph Optimization also plays an essential role in state-of-the-art SLAM tasks as a back-end optimizer, for example as with distributed mapping \citep{Choudhary2017DistributedMW} and rotation estimation \citep{PGOSurvey_Luca}. Energy-efficient accelerator for VIO in \citep{karaman_droneVIO,karaman_miniVIO} also enables the localization and mapping on miniaturized robots. Several other works~\citep{karaman_sparsetoDense,scaramuzza_eventCameras,scaramuzza_motionEstimation} provide a multitude of techniques ranging from specialized visual sensing capability to estimation of depth and motion in the view with monocular system.
% PGO~\citep{PGOSurvey_Luca,LucaMultiRobotPGO}, VIO~\citep{karaman_droneVIO,karaman_miniVIO}, and several other techniques~\citep{karaman_sparsetoDense,scaramuzza_eventCameras,scaramuzza_motionEstimation}. 
% \subsection{Challenges}
% To achieve accurate AoA estimation on mobile platform with arbitrary trajectory, there are several challenges we mainly settle in this work. Firstly, characterizing the impact of trajectory geometry is important such as informativeness, ambiguities. Given an arbitrary trajectory with ground and aerial platform, we want to find out the performance of them in our system. Secondly, We need take into account mobility on both ends which has been considered a hard problem because difference dynamic on both sides would results in indeterminate change in  wireless signal. Finally, there are noise and carrier frequency offset(CFO) from using different radios on all communicating agents. Not addressing the CFO in transmitter and receiver would lead to mismatch in frequency and fail the SAR algorithm. 
\subsubsection*{\textbf{Antenna array theory:}}
Traditional antenna arrays that provide AOA information are often bulky and hence not suitable for small agile robot platforms~\citep{Bjrnson2019MassiveMI}. To this end, we consider a SAR inspired approach that uses robot motion and signal measurements over several communicated packets, to obtain a full AOA profile.
% 3D SAR necessitates an analysis of arbitrary shaped antenna array in order to evaluate its performance. 
This paper builds closely off of antenna array theory in order to characterize AOA performance metrics resulting from 3D SAR applied arbitrary robot trajectory in 3D space.
The Cramer Rao Bound (CRB) is a often utilized tool for the performance analysis of different antenna array geometries\citep{Gazzah2006CramerRaoBF,Mirkin1991CramerRaoBO}. Specifically, the CRB provides important lower bounds estimates on the variance of the resulting angle-of-arrival estimates as a function of antenna array geometry~\citep{Moriya2012CRLB3D,Mohamed2019ASO}; in other words, CRB analysis \emph{reveals the relationship between the robot trajectory and the richness of information attainable from processing received communication signals}. This key observation opens the possibility of thinking of SAR as an enabling technology for a new kind of \emph{sensing} for robotics. 
\vspace{12pt}

Thus, in comparison to previous work done in SAR, our proposed system is a generalized formulation of a direction finding capability for robots that combines local trajectory estimation methods with antenna array theory. It enables a robot to obtain relative AOA of a WiFi signal transmitter (stationary or moving) by using arbitrary 3D motion. However, this requires a mathematical, algorithmic, and experimental framework for characterizing the impact of i) 3D trajectories on the informativeness (or richness of information) derived from processing collected WiFi signals, ii) error in trajectory estimation on the resulting accuracy of the AOA estimates, and iii) mobility at \emph{both ends} meaning mobility of both the transmitting and receiving robots, in order to enable continuous data collection that is most compatible with general multi-robot tasks.  We address these objectives in the current paper.
% \subsection{Robotics Wireless Sensor Networks (RWSN)}
% Usage of wireless signals have been explored in robotics predominantly for optimizing communication network in multi-robot systems. Such sensor networks i.e \emph{RWSN}~\citep{Ghosh2019RoboticWS} typically rely on controlled movement of robots to prioritize communication maximization and are expected to guarantee certain communication requirements~\citep{Ghosh2019RoboticWS}. Previous work done in this domain for multi-robot coordination using Wi-Fi requires information relay~\citep{Kantaros2014CommunicationawareCC,Ny2012AdaptiveCD}, a fixed radio station~\citep{Ghaffarkhah2012PathPF,Yan2014EfficientCD} or creating signal strength maps~\citep{Hsieh2007AdaptiveTO,Hsieh2004ConstructingRS}. WiFi has also been used for mapping application~\citep{Mostofi2010CompressiveCO,Karanam20173DTI,GonzalezRuiz2014AnIF}. Majority of RWSN based approaches use Received Signal Strength (RSS) which refers to the power of the signal. 

% This paper explores the use of Wi-Fi to explicitly \emph{sense neighboring robots without any constraints on motion}. without the need to satisfy communication requirements or generate maps. Our method relies on minimal communication between robots and leverages the physical properties of wireless signal to enable coordination. As RSS is coarse, and hence ill-suited for extracting spatial information with accuracy and precision~\citep{?}, we use \emph{Channel State Information} (CSI) - information obtained from PHY layer of 802.11 protocol. CSI essentially facilitates capturing the phase change of wireless signal. It thus provides more granularity compared to RSS and thus results in higher AOA precision~\citep{Yang2013FromRT,Ma2019WiFiSW}.

% \subsection{Synthetic Aperture Radar and Angle-of-Arrival}
% Traditionally, using Wi-Fi signals to obtain AOA has been used for localization, like in~\citep{Xiong2013ArrayTrackAF} which uses large antenna arrays, and in~\citep{Kotaru2015SpotFiDL} which requires a static setup of antenna routers. Similarly, other works in robotics that specifically use AOA information for the mobility of all the robots in the team~\citep{Karanam2018MagnitudeBasedAE}, or depend on bulky hardware which would be difficult to deploy on aerial robots~\citep{Min2018ADA}. Such methods are generally infeasible for robotic platforms due to restriction on size and more importantly, requirement for mobility. To address the challenge of size constraint, we deploy our system using commodity Wi-Fi cards which are ubiquitous to robotic platforms. In order for our system to be compatible with mobile platforms, we use
% Synthetic Aperture Radar (SAR) inspired approach, a sensing modality that has been applied in a variety of contexts, including satellites~\citep{Krieger2006SpaceSAR}, RADAR imaging~\citep{Chauhan1991RADARSAR}, and most recently, for mobile wireless applications~\citep{Kumar2014AccurateIL}. 
% % Most related to our work is SAR in the context of WiFi, since WiFi is readily available upon drones. 

% A combined use of SAR and Wi-Fi has been shown to be useful for applications including adaptive robotic networks~\citep{Gil2015AdaptiveCI}, Simultaneous Localization and Mapping~\citep{Wang2019ActiveRF}, materials sensing~\citep{Zhang2019OnTF}, localization~\citep{Vasisht2016DecimeterLevelLW} and through-wall sensing~\citep{Adib2015ThroughWall}. Multi-robot coordination approaches using AOA information either require performing specific motion (e.g. rotation) to address the limited field of view problem using monocular camera~\citep{Franchi2012ModelingAC} or run in simulated environment~\citep{Zhelo2018CuriositydrivenEF}~\citep{Parasuraman2018ConsensusCO}. We distinguish ourselves from existing work in the space due to our ability to support an \emph{arbitrary path}, rather than a pre-defined path or an orbit and validating our approach on real hardware.

% \subsection{Visual Inertial Odometry}
% Since our approach requires accurate position estimates of the Wi-Fi antenna attached to a robot, one of the factors that influence relative AOA between mobile robots, is the trajectory estimation obtained from an on-board sensor. While previous work has successfully shown how an IMU sensor can be used for this purpose~\citep{Wang2019ActiveRF},\citep{Kumar2014AccurateIL}, it is limited in terms of mobility. In this paper, we leverage an off-the-shelf on-board camera sensor running a \emph{Visual Inertial Odometry}(VIO) system to obtain robot's pose estimates~\citep{Tracking_camera}, on account of its size and ease of use. To the best of our knowledge ours is the first system that combines trajectory estimation from a camera with information from wireless signals to obtain relative AOA between two robots. We emphasize that any on-board sensor that can provide accurate local pose estimates would be compatible with our system. For a camera sensor, our approach is not restricted to any specific trajectory estimation algorithm and can be used as is with other methods~\citep{Qin2017VINSMonoAR,Rosinol2019KimeraAO}.


% \begin{enumerate}
% 	\item General references about multi-robot systems, coordination, and shared info between agents
% 	%\edit{Stephanie mentioned wanting to include a UWB TOF paper but I'm not sure where that would be appropriate to tie in.}
% 	%\edit{Diana + Swarun}
% 	\item %Cramer Rao Bound for error analysis\edit{Diana + Swarun}
% 	\item %Cramer Rao Bound for error analysis\edit{Diana + Swarun}
% 	\item Coverage
% 	\item Frontier exploration
% 	\item Optical flow
% 	\item SLAM and ORB-SLAM
% \end{enumerate}


==> text/results.tex <==
\section{Results}\label{sec:results}
In this section we present the results of extensive simulation and hardware experiment studies that demonstrate agreement of practical implementations with the development and analysis sections  of the paper. In particular we study 1) the feasibility of attaining accurate AOA profiles $F_{ij}(\phi,\theta)$ using relative trajectory of a receiving robot in the moving ends case where both transmitting and receiving robots are simultaneously mobile, 2) the informativeness of different trajectory geometries in 2D and 3D, and 3) the impact of trajectory estimation errors on attainable $AOA_{max}$ accuracy. We find that:
\begin{itemize}
    \item Our developed framework from Section~\ref{sec:moving_ends} solves the \emph{moving ends} problem where $F_{ij}(\phi,\theta)$ is attainable even when both the transmitting and receiving robots are simultaneously moving. Furthermore in this case, \emph{relative} trajectories being more informative lead to higher accuracy of $F_{ij}(\phi,\theta)$.
    % \item 3D robot trajectories lead to AOA estimates that are \edit{$X\%$} more accurate on average than those produced by 2D trajectories (curved or linear), and that \emph{informativeness} as derived in Section~\ref{sec:characterization-trajectory-err-analysis} is a good predictor of an accurate AOA profile based on trajectory geometry.
    \item Arbitrary 3D trajectories generate highly accurate $F_{ij}(\phi,\theta)$ (less than 10 $\deg$ error in $AOA_{max}$ for 95\% of trials). In contrast, planar 2D curved and linear trajectories only 50\% and 7\% of trials show error below 10 $\deg$ respectively.
    \item For robot trajectory estimates with an average of $5\%$ estimation error obtained using an on-board Intel RealSense T265 Tracking camera (0.06m error in position over 1.2m long trajectories), attainable $AOA_{max}$ estimation accuracy was shown to be within 10.03 degrees in azimuth and 2.23 degrees in elevation on average. 
\end{itemize}

We subsequently describe our experimental setup in section \ref{sec:result_exp_setup}. The results for moving ends experiments are detailed in section \ref{sec:results_movingEnds}. Section \ref{sec:results_informativeness} and \ref{sec:results_traj_erro_AOA} show the results for trajectory informativeness and the impact of trajectory estimation respectively.  

\subsection{Experimental setup} \label{sec:result_exp_setup}
\subsubsection*{\textbf{Testbed and hardware setup:}} We use an off-the-shelf \emph{Turtlebot3 Waffle} for our ground robot and an \emph{NXP KIT-HGDRONEK66} drone for our aerial robot (Fig.~\ref{fig:hardware_robots}). Each robot is mounted with a lightweight 2 DBi omnidirectional WiFi antenna, \emph{UP Squared} on-board computer which uses an Intel 5300 WiFi module and an out-of-the-box \emph{Intel Realsense T265} tracking camera which gives local pose estimates at 200 Hz. We evaluate our system in a 10,000 square feet, 23-foot-tall indoor environment. Using 105 cameras, the \emph{Optitrack} motion capture system deployed in the testbed provides groundtruth measurements for robot trajectories and relative AOA between them. Using groundtruth trajectories, we first obtain a benchmark performance for our system. A second set of experiments using Intel Realsense T265 tracking camera trajectories is conducted to understand how $F_{ij}(\phi,\theta)$ and $AOA_{max}$ are impacted when using position information from VIO systems since they have become ubiquitous to mobile robot platforms in recent years.
%====Moving ends results 3D Traj====
\begin{figure}
	\centering
    \includegraphics[width=8.0cm,height=8.0cm]{Images/Relative_3D_Traj_results.PNG}
	\caption{\footnotesize{\emph{(a) Hardware experiment showing the 3D trajectory for UAV $\boldmath{\chi_i}\textbf{(t)}$ and the corresponding relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ due to motion of transmitting robot $j$ with trajectory $\boldmath{\chi_j}\textbf{(t)}$. Our approach for moving ends gives similar profile results for 3D trajectories as seen in Fig.~\ref{fig:3D_SAR_AOA}. (b) AOA profile showing true Angle-Of-Arrival ($\phi_g$, $\theta_g$) = (\ang{90}, \ang{91}), denoted by red 'x' in the profiles.}}}
	\label{fig:Relative_Traj_comparison_3D}
\end{figure}
%====Moving ends results 3D Traj====

For experiments with groundtruth trajectories the center of the rigid body model generated by motion capture system is aligned with the physical placement of WiFi antenna on the robots' chassis. For experiments with tracking camera trajectories, the antenna and T265 camera are aligned on the robots' chassis and their offset, if any, is accounted for. The robots use minimal communication (broadcasting ping packets) over the center frequency channel of 802.11 5GHz band. The total data transmission overhead for our system amounts to a maximum of 15 kB in 3 seconds when a receiving robot performs 3D SAR. Note that the frequency of such transmission would highly depend on the application. In our dynamic rendezvous hardware application (Sec. \ref{sec:hardware_application}), as the receiving robot continuously requires $AOA_{max}$ for navigation, this leads to an average 5kB/s transmission overhead. This includes phase information collected from transmitted signals between robots and local position estimates from neighboring robots (in their own coordinate frame). 

Pose estimates from the tracking camera and channel information from transmitted signals are collected using each robots' on-board computer. The current nature of our code-base requires processing the data on an off-board computer but the computation requirements for our system are satisfied by on-board computer as well. All processing is done in real time. We use both Bartlett and MUSIC estimators~\citep{Krim1996TwoDO} for generating $F_{ij}(\phi,\theta)$ and our results indicate which estimator was used. We note that our theoretical analysis in Section~\ref{sec:characterization-trajectory-err-analysis} uses a Bartlett formulation and thus all trajectory error experiments (Sec. \ref{sec:results_traj_erro_AOA}) were conducted using the Bartlett estimator.

\subsubsection*{\textbf{Software setup:}} We use Ubuntu 16.04 with kernel 4.15, as the OS for the on-board computer. It runs the following: Drone control that uses ROS and MAVROS, pose estimation from realsense libraries for the tracking camera\endnote{Code samples used for T265 tracking camera to get position estimates can be found in their github repository : https://github.com/IntelRealSense/librealsense} and a modified iwlwifi driver with 802.11 CSI toolbox~\citep{Halperin_csitool} that collects wireless channel state information (CSI), which is used to calculate signal phase. The AOA profile is calculated in an off-board fashion using a laptop that runs a Matlab framework. As per our assumption, global clock synchronization among the robots is achieved by running ntpd at the start an experiment. 
%\subsection{Simulation Results for Cramer Rao Bound Error vs. Geometry (curvature)}
% \subsection{Simulation Results for Cramer Rao Bound Error for robot trajectory}
% %\edit{Diana + Swarun}
% \subsection{Simulation Results for predicted AOA error vs. Trajectory error}
% Note: Review if this section is going in or not.
% %\edit{Diana + Swarun}
%====Moving ends 2D results====
\begin{figure}
	\centering
    \includegraphics[width=8.5cm,height=7.5cm]{Images/Relative_2D_Traj_results.PNG}
	\caption{\footnotesize{\emph{(a) Hardware experiment showing linear 2D trajectory $\boldmath{\chi_i}\textbf{(t)}$ for signal receiving robot $i$ and the corresponding curved relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ due to motion of transmitting robot $j$ with trajectory $\boldmath{\chi_{j}}\textbf{(t)}$. Using the relative trajectory, our approach for moving ends (Sec. \ref{sec:moving_ends}) gives similar profile results for 2D curved trajectories (Fig.~\ref{fig:3D_SAR_AOA}) with ambiguity only along elevation angle. (b) AOA profile showing ($\hat{\phi}$, $\hat{\theta}$) = (\ang{-90}, \ang{73}) while true AOA ($\phi_g$, $\theta_g$)  = (\ang{-90}, \ang{90}), denoted by red 'x' in the profiles. Relative trajectory $\boldmath{\chi_{ij}}\textbf{(t)}$ (curved 2D) thus has a more informative geometry than actual trajectory $\boldmath{\chi_i}\textbf{(t)}$ (linear 2D).}}}
	\label{fig:Relative_Traj_comparison_2D}
\end{figure}
%====Moving ends 2D results====

\subsection{Moving ends}\label{sec:results_movingEnds}
Our SAR development allows for generating AOA profile $F_{ij}(\phi,\theta)$ using arbitrary 3D trajectories for a static transmitting robot (Sec. \ref{sec:Development}). Extending that formulation to the \emph{moving ends problem}, in this section we demonstrate the accuracy of the resulting $F_{ij}(\phi,\theta)$ obtained using relative trajectory $\boldmath{\chi_{ij}\textbf{(t)}}$ with mobile receiving and transmitting robots $i$ and $j$. Relative trajectory can be obtained using different onboard sensors, however for proof-of-concept purposes of our developed framework, we provide position estimates of local robot trajectories using an external motion capture system. The following scenarios are evaluated:
\begin{enumerate}
     \item Robot $i$ performs a helix motion at 0.5 m/s (Fig.~\ref{fig:Relative_Traj_comparison_3D})
     \item Robot $i$ performs a linear motion at 0.1 m/s (Fig.~\ref{fig:Relative_Traj_comparison_2D})
\end{enumerate}
and the transmitting robot $j$ moves along a linear trajectory with varying speed (max speed of 0.1m/s), and is at a distance of 10 meters from robot $i$. Results for the 3D scenario using a sample trajectory from hardware experiments are shown in Fig.~\ref{fig:Relative_Traj_comparison_3D}. We see that $F_{ij}(\phi,\theta)$ obtained using relative trajectories for a moving transmitting robot show similar behavior when compared to those obtained for a static transmitting robot (Fig. \ref{fig:3D_SAR_AOA}).

We make interesting observations with respect to the use of relative trajectories. For example, when the transmitting and receiving robots are moving linearly along different directions and with different speeds, the relative trajectory obtained has a curved geometry which eliminates ambiguities along $\phi$ (Fig. \ref{fig:Relative_Traj_comparison_2D}). Thus, we postulate that depending on the direction and variation in speed of the moving robots, more informative and less ambiguous trajectories can be naturally obtained.  Further investigation of this observation, namely, exploiting relative trajectories for obtaining higher informativeness from 2D trajectories, is an interesting avenue for further research. Results pertaining the informativeness of different trajectory geometries are discussed in the following section.
%=====CRB and AOA error 2D vs 3D==
\begin{figure}
    %\includegraphics[scale=0.3]{CRB_Schematic.png}
    \includegraphics[width=8.5cm,height=6.0cm]{Images/CRB_AOA_error_2D_vs_3D.png}
    %\vspace*{-0.2in}
    \caption{\footnotesize{\emph{Aggregate results comparing 2D and 3D trajectories obtained from hardware experiments in terms of $AOA_{Error}$ (Eqn.~\ref{eqn:AOA_euclidean_error}) and Cramer-Rao bound. A low of value of CRB indicates that the trajectory has high informativeness. From the distribution of CRB and AOA error for 2D and 3D trajectories, 3D trajectories have a lower $AOA_{Error}$ on account of being more informative than 2D trajectories.}}}
    \label{fig:CRB_vs_AOA_error}
\end{figure}
%=====CRB and AOA error 2D vs 3D==
%====Ambiguity of different trajectories====
\begin{figure*}
	\centering
        \includegraphics[width=16.3cm,height=9.0cm]{Images/Informativeness_differentTrajectories_v2.png}
    	\caption{\footnotesize{\emph{Shows different trajectories (left) obtained from hardware experiments and ambiguities in the AOA profile $F_{ij}(\phi,\theta)$ (right). True AOA ( $\phi_g$, $\theta_g$) = ( $\ang{-90}$, $\ang{91}$) to the WiFi signal source (i.e transmitting robot) is denoted by red 'x' in the profiles. 3D trajectories have higher informativeness and have no ambiguities in the AOA profile (top right).}}}
    	\label{fig:Traj_ambiguity}
\end{figure*}
%====Ambiguity of different trajectories====
%====AOA error distribution====
\begin{figure}
        \includegraphics[width=8.5cm,height=6.0cm]{Images/aoa_distribution.png}
        \caption{\footnotesize{\emph{Aggregate benchmark results using groundtruth trajectories that show AOA error in azimuth angle $\phi$ and elevation angle $\theta$ (Defn. \ref{def:AoA-error}). The profiles are generated for 101 hardware experiment trials each for the three trajectory types (2D linear, 2D curved and arbitrary 3D). 3D trajectories (green) have higher AOA accuracy in both azimuth $(\phi)$ and elevation $(\theta)$ directions as compared to 2D trajectories, which show high error in $\theta$ (curved trajectory). Moreover 2D linear trajectories have additional errors in $\phi$. Thus, the aggregate results align with those shown in Fig. \ref{fig:Traj_ambiguity} for individual samples of each trajectory type.}}}
        \label{fig:Different_mocap_Traj_comparison_AOA_error}
        \vspace{-10pt}
\end{figure}
%====AOA error distribution====
%====CDF plots====
\begin{figure*}
	\centering
    \includegraphics[width=15.0cm,height=8.0cm]{Images/CDF_AOA_phi_theta_error.png}
	\caption{\footnotesize{\emph{Benchmark results obtained using groundtruth trajectories for a receiving robot in hardware experiments. The transmitting robot is at a distance of 10m. (a) CDF plot for $AOA_{Error}$ error for 101 trials of each trajectory type (linear, curved and arbitrary 3D). 3D trajectories have the lowest $AOA_{Error}$ (Defn. \ref{def:AoA-error}) which is less than $\ang{10}$ for 95\% of trials. For planar 2D curved and linear trajectories only 50\% and 7\% of trials show error below \ang{10} respectively. (b) and (c) show the individual CDF plots for AOA error in $\phi$ and $\theta$ respectively. 2D linear trajectories have the highest error overall. We note that even groundtruth trajectories incur AOA error due to factors mentioned in Sec. \ref{sec:ps_trajectory_impact}}.}}
    \label{fig:CDF_phi_theta}
\end{figure*}
%====CDF plots====

\subsection{Informativeness of 2D and 3D trajectories}\label{sec:results_informativeness}
In this set of experiments our objective is to study the impact of trajectory geometry on $AOA_{max}$ estimation. In order to isolate the effect of trajectory geometry from other factors such as position estimation errors, the results of this section use groundtruth robot trajectories obtained from motion capture (the effect of position estimation errors is studied subsequently in Section~\ref{sec:results_traj_erro_AOA}). For a single experiment, relative $AOA_{max}$ is computed between a static ground robot (signal transmitting) and a signal receiving robot moving along a trajectory of one of the following three types - 2D linear trajectory, 2D curved trajectory and 3D arbitrary trajectory (See Fig. \ref{fig:Traj_ambiguity}). We call such an experiment a \emph{trial} and conduct a total of 101 \emph{trials} for each type of trajectory. For this set of experiments the robots are separated by a distance of 10m and are in line-of-sight of each other to exclude other impacting factors. The application of our system to non-line-of-sight scenarios is studied subsequently in Section~\ref{sec:hardware_application}.

We note that informativeness is defined in both the azimuth and elevation directions and while 3D trajectories demonstrate high informativeness in both directions, 2D curved trajectories perform better in azimuth ($\phi$) and worse in elevation ($\theta$).  Fig.~(\ref{fig:CRB_vs_AOA_error}) demonstrates that the \emph{informativeness} calculated for each trajectory (inverse of the CRB) successfully captures this improved performance in $AOA_{Error}$ for 3D versus 2D trajectories. This provides empirical evidence of the analysis derived in Section~\ref{sec:cr-bound} which predicts higher informativeness (smaller attainable CRB) for 3D trajectories. Fig.~(\ref{fig:CDF_phi_theta}) shows the aggregate performance over 101 trials of each of three different trajectory types: 2D linear, 2D curved, and 3D.  Overall $AOA_{Error}$ (Fig.~\ref{fig:CDF_phi_theta} (a)) is significantly lower for 3D trajectories as compared to its 2D counterparts. Specifically, 3D trajectories demonstrate less than $\ang{10}$ $AOA_{Error}$ for 95\% of the total trajectory samples within the same type, where as only 50\% of 2D curved trajectories and 7\% of 2D linear trajectories show similar accuracy. This trend is again shown empirically in our application scenario results in Section~\ref{sec:hardware_application}.
%====Error in AOA vs ATE==
\begin{figure}
		\centering
        \includegraphics[width=7.5cm,height=5.5cm]{Images/ATE_error_vs_aoa_beta_error_addNoise_to_a_singelMOcap_traj.png}
        \caption{\footnotesize{\emph{Simulation Results showing Angle-Of-Arrival estimation error vs Absolute Trajectory error in translation ($ATE_{trans}$: Eqn. \ref{eq:ATEtran}). Trajectory error is added using simulated noise to a groundtruth trajectory of receiving robot obtained in hardware experiments. The range of $ATE_{trans}$ on X-axis reflects the observed error in Intel Realsense T265 tracking camera trajectories (Fig. \ref{fig:ATE_trans_error_cameraTraj}).}}} 
    	\label{fig:aoa_vs_ATE_error}
\end{figure}
%====Error in AOA vs ATE==

Hardware results also reveal important intuition behind the informativeness of different trajectory geometries. Fig.~(\ref{fig:Traj_ambiguity}) demonstrates a typical trial for each of the three trajectory types studied in this paper. Here it is shown that for trajectory types of lower informativeness such as the linear 2D trajectory, ambiguities are observed in $F_{ij}(\phi,\theta)$ for relative direction $(\hat{\phi}, \hat{\theta})$ of the transmitting robot. This is due to the inability of the linear antenna array geometry traced by receiving robot to uniquely distinguish a transmitting robot's location for certain direction tuples $(\phi,\theta)$ using phase differences. This problem is greatly alleviated by using trajectories with high levels of informativeness (3D trajectories). 

In conclusion, our results clearly indicate that 3D trajectories have the highest informativeness amongst all trajectory types studied, resulting in more accurate estimation of $AOA_{max}$ in both azimuth and elevation, as predicted by the analysis from Section~\ref{sec:Analysis_impact_factors}.

% \noindent \textcolor{red}{In figure \ref{Fig:Different_mocap_Traj_comparison}, we collected total 25 samples by letting robots moving along three types of trajectory we just described to demonstrate the accuracy of our approach. The static robot is placed more than 15 meters away from robot which is performing movement.  In scatter Figure \ref{fig:Different_mocap_Traj_comparison}, 3D helix-like trajectory provides the most accurate AOA whose ground truth error maintain below 5 degrees in $\phi$ and 8 degrees in $\theta$.
% }
% %====Simulation Error in AOA vs YAW==
% \begin{figure}
% 		\centering
%         \includegraphics[width=7.5cm,height=5.5cm]{Images/Yaw_error_vs_aoa_beta_error_addNoise_to_a_singelMOcap_traj.png}
%     	\caption{\footnotesize{\emph{Results for Angle-of-Arrival estimation error in azimuth vs yaw error in UAV 3D trajectory. To study the impact of trajectory error independently, we add simulated noise to single oracle trajectory obtained from hardware experiments. The yaw error accumulation results in similar error or "shift" in $\phi$ (see section~\ref{sec:characterization-trajectory-err-analysis}). }}}
%     	\label{fig:Aggregate_AOA_error_vs_mean_yaw}
% \end{figure}
% %===Simulation Error in AOA vs YAW=======

\subsection{Effect of trajectory estimation error on AOA}\label{sec:results_traj_erro_AOA}
% In this section, we evaluate our system accuracy for AOA estimation based on two sources of error in trajectory estimation. First we detail the results for AOA estimation error (Defn.~\ref{def:AoA-estimation-error}) in presence of trajectory estimation error. Next, we show results for the impact of trajectory discretization on the AOA profile. 
% \subsubsection{Impact of Trajectory estimation error:}\label{sec:traj_error_impact_results}
As computing AOA profiles $F_{ij}(\phi,\theta)$ requires knowing a robot's local displacement and most robots in the field rely on onboard sensors to estimate their position, in this section we experimentally study the impact of trajectory estimation on $F_{ij}(\phi,\theta)$. We do so by measuring the $AOA_{max}$ (maximum magnitude path in $F_{ij}(\phi,\theta)$) accuracy in presence of trajectory estimation errors. Our empirical analysis includes both a simulation and a hardware component where the simulation provides a controlled study in which noise can be added systematically to reveal error trends, and the hardware component provides aggregate results showing the impact of trajectory estimation error on $AOA_{max}$ accuracy in an actual all on-board sensing robot system. For the hardware experiments we use trajectory estimates provided ``out-of-the-box'' from the tracking camera. No additional optimization techniques were used to improve trajectory estimation though we do note that it is possible to obtain better trajectory estimation using state-of-the-art methods and sensors (See Sec. \ref{sec:related_works}). The $AOA_{max}$ estimates obtained are compared against benchmark results from using groundtruth trajectories (obtained from motion capture system). 
%====Error in Camera Traj ===
\begin{figure}
		\centering
        \includegraphics[width=8.3cm,height=5.2cm]{Images/ATE_error_cameraTraj.png}
        \caption{\footnotesize{\emph{Absolute Trajectory Error ($ATE_{trans}$: Eqn. 7) observed for Intel Realsense T265 tracking camera trajectories obtained from our hardware experiments.}}}
    	\label{fig:ATE_trans_error_cameraTraj}
\end{figure}
%====Error in Camera Traj ===
%========Mocap_Vs_camera_aggregate=======
\begin{figure*}
	\centering
	\begin{minipage}{.45\linewidth}
         \includegraphics[width=8.0cm,height=5.5cm]{Images/Mocap_vs_camera_AOA.png}
	\end{minipage}
	\hspace{6pt}
	\begin{minipage}{.45\linewidth}
        \includegraphics[width=8.0cm,height=5.5cm]{Images/Mocap_vs_camera_AOA_theta.png}
	\end{minipage}
    \caption{\footnotesize{\emph{Aggregate results of AOA estimation for 59 hardware experiments. Each experiment records the Intel Realsense T265 tracking camera trajectory and groundtruth for the receiving robot along with their respective $F_{ij}(\phi,\theta)$. Groundtruth AOA $(\phi_g, \theta_g)$ = ( $\ang{0}$, $\ang{91}$). Sub-plot on the left shows error in $\phi$ with mean = -0.63 degrees for groundtruth trajectory and -10.03 degrees for tracking camera trajectory. Sub-plot on the right shows error in $\theta$ with mean = -0.69 degrees for groundtruth trajectory and 2.23 degrees for tracking camera trajectory. Thus, with high error in estimated trajectory, the corresponding AOA accuracy is low, compared to that obtained from groundtruth trajectory. \textcolor{red}{check with WSR toolbox paper results. set KDE plot common_norm=False.}}}}
    \label{fig:Mocap_vs_camera_AOA}
\end{figure*}
%========Mocap_Vs_camera_aggregate=======
\subsubsection{\textbf{Simulation study:}} Our simulation study emulates accumulating error in trajectory estimates in the following way: we generate multiple noisy trajectories $\boldmath{\hat{\chi_i}}\textbf{(t)}$ by adding accumulating Gaussian noise to a sample 3D groundtruth trajectory $\boldmath{\chi_i}\textbf{(t)}$ of the receiving robot $i$. $F_{ij}(\phi,\theta)$ is then generated for these $\boldmath{\hat{\chi_i}}\textbf{(t)}$ to obtain an $AOA_{max}$ estimate $(\hat{\phi},\hat{\theta}$) which is then compared with the true simulated AOA direction $(\phi_g,\theta_g)$ to compute AOA error (cf. Defn.~\ref{def:AoA-error}).

In order to generate an $F_{ij}(\phi,\theta)$ (cf. Eqn.~\eqref{eqn:bartlett_estimator_fin}) using simulated noisy trajectories as described above, we must also simulate the wireless channel $\mathbf{h_{ij}(t)}$ from the static transmitting robot $j$, obtained over these trajectories i.e over $\boldmath{\hat{\chi_{i}}\textbf{(t)}}$. 
To simulate the wireless channel, we fix the virtual location $\hat{p_j}(t_k)$ of static $j$ at 10m from position $p_i(t_{k})$ in $\boldmath{\chi_i}\textbf{(t)}$. For any position $p_i(t)$, $t \in [t_{k},\hdots,t_{l}]$ where $k$=0, $l$=500 and $d_{ij}(t)$ is the distance between $p_i(t)$ and $p_j(t_k)$, the channel measurements $h_{ij}(t)$ can thus be simulated from Eqn. \ref{eqn:channel_basic_eqn} to obtain $\bold{h_{ij}(t)}$. As $AOA_{max}$ captures relative angle information, we simulate noise in $\boldmath{\chi_i}\textbf{(t)}$ by applying increasing cumulative angular error in $\varphi_i(t)$ and $\xi_i(t)$ for each $p_i(t)$ (is represented in polar coordinates) in $\boldmath{\chi_i}\textbf{(t)}$. We assume that the errors for position ($x_i(t)$, $y_i(t)$, $z_i(t)$) in Cartesian coordinates are translated to errors in $\varphi_i(t)$ and $\xi_i(t)$ only in the corresponding Spherical coordinates.

$\boldmath{\hat{\chi_{i}}\textbf{(t)}}$ are simulated in such a way that their $ATE_{trans}$ error (cf. Eqn.~\eqref{eq:ATEtran}) are representative of those characteristic from using on-board sensors. This is based on our observations of estimation error using tracking camera (see Fig. \ref{fig:ATE_trans_error_cameraTraj}). In particular, to generate the first noisy trajectory, for each position $p_i(t)$ in $\boldmath{\chi_i}\textbf{(t)}$, we sample angular error (in degrees) from a Gaussian distribution. This is then repeated for all $\hat{p_i}(t)$, with the errors being cumulatively added for successive positions. The noise is simulated in a way that the accumulating error in the trajectory would reflect realistic ATE as we obtained in Fig.~\ref{fig:ATE_trans_error_cameraTraj} from the tracking camera on the drone. This generates $\boldmath{\hat{\chi_{i}}\textbf{(t)}}$ from $\boldmath{\chi_i}\textbf{(t)}$ with an accumulating angular drift. The corresponding $ATE_{trans}$ error for $\boldmath{\hat{\chi_{i}}\textbf{(t)}}$ then is obtained by converting the noisy trajectory positions $\hat{p_i}(t)$ from spherical coordinates to Cartesian coordinates and then using Eqn.~\ref{eq:ATEtran}. To generate additional noisy trajectories, we increase the sampled angular error for each successive simulated trajectory steadily so that the $ATE_{trans}$ error ranges from 0.02m to 0.12m. A total of 50 noisy trajectories are generated. 

Our empirical results support our analytical development from \emph{Lemma} 2 and 3 (Sec. \ref{sec:characterization-trajectory-err-analysis}).
% where we see that an increasing azimuth error in the trajectory produces a shift (linear increase) in estimated AOA error in azimuth ($\phi$) as shown in Fig.~\ref{fig:Aggregate_AOA_error_vs_mean_yaw}. A similar trend is observed for elevation error and AOA $\theta$ estimation error. 
The corresponding $ATE_{trans}$ error generated for simulated trajectories also shows a increasing linear relationship with AOA error (Fig.~\ref{fig:aoa_vs_ATE_error}). Thus we conclude that trajectories with $ATE_{trans}$ in the range (0.02, 0.12) will demonstrate an AOA estimation error in the range (2,10) degrees in the absence of other factors that impact $F_{ij}(\phi,\theta)$.

\subsubsection{\textbf{Hardware experiments:}} For hardware experiments, we compare $AOA_{max}$ estimation using pose estimates obtained from Intel Realsense T265 tracking camera against benchmark $AOA_{max}$ estimates obtained from groundtruth robot trajectories. Both trajectory types are simultaneously collected for the receiving robot using the tracking camera (mounted on the aerial robot) and an external motion capture system. $AOA_{max}$ estimates are calculated in realtime, while keeping the transmitting robot static (results involving a mobile transmitting robot are presented in Section~\ref{sec:results_movingEnds} and Section~\ref{sec:hardware_application}). Average robot trajectory lengths are 1.2m per AOA profile generated. Fig.~(\ref{fig:Mocap_vs_camera_AOA}) shows a Kernel Density Estimation (KDE) distribution plot comparing AOA estimation error in $\phi$ and $\theta$ for 59 trajectories using position estimates obtained via tracking camera trajectories versus the benchmark (obtained using groundtruth trajectories). The error mean in azimuth angle $\phi$ and elevation angle $\theta$ is -0.63 degrees, -0.69 degrees respectively for groundtruth trajectories, and -10.03 degrees, 2.23 degrees respectively for tracking camera trajectories. Fig.~\ref{fig:ATE_trans_error_cameraTraj} shows an mean error of 0.06m for tracking camera trajectories which were 1.2m long on average. Thus the results shown in Fig.~\ref{fig:Mocap_vs_camera_AOA} represent average $AOA_{max}$ estimation error for trajectories with an average of 5.0\% estimation error. We note that our benchmark results represent an empirical lower bound for $AOA_{max}$ estimation error attainable using robot trajectory estimation techniques with improved position estimation accuracy in the presence of other factors (e.g. trajectory geometry) that impact $F_{ij}(\phi,\theta)$.

% \subsection{Impact Of Discretization and inter-pose spacing}\label{sec:inter-element-spacing-HWresults}

% \subsubsection{Impact of Trajectory Discretization:}\label{sec:discretization_impact_results}
% Following the analytical development in section~\ref{sec:Inter-pose_spacing_lemma}, we conduct numerical analysis of Eqn.~\ref{eqn:main_term_separate} for increasing inter-element separation for a idealized case of 2D circular trajectory to understand how it impacts AOA estimation. As seen in Fig.~\ref{fig:Inter_element_spacing_numerical_results}, with increased discretization , anomalous peaks start to dominate the AoA profile. \edit{As simulated channels (Eqn.~\ref{eqn:Simulated_CSI}) are used for the theoretical analysis, we do not need to multiply forward-reverse channels to cancel out phase offset and it suffices to use the forward channel as given in Eqn.~\ref{eqn:forward-reverse-sim}}. The threshold for which such anomalous peaks start to become evident is $\frac{\lambda}{2}$, where $\lambda$ is the wavelength. This trend is independent of the radius of the circular array. Thus increased spacing results in the a noisier AOA profile, making it difficult to discern the true AOA peak from other anomalous peaks. Similar observations are seen in hardware experiments. Note that we calculate the percentage violations of inter-pose spacing being greater than $\frac{\lambda}{4}$ (as the real wireless channels are modelled using Eqn.~\ref{channel_forward_revese_prod} to cancel phase offset, section~\ref{sec:Development}) as seen in Fig.~\ref{fig:Bad_element_percent_allOnBoard}. 
% Results of wireless signal profile for one such hardware trial that compares motion capture and tracking camera trajectories are shown in Fig.~\ref{fig:hW_results_inter-element_distance_AOA_mocap_vs_camera}. The AOA profile with higher percentage of such violations (camera trajectory) is much more noisier. Note that these results are also impacted other factors that have been analyzed independently (section~\ref{sec:Analysis_impact_factors}), leading to incorrect AOA estimation.
% \subsection{Results for moving ends experiments}
% %========Mocap_Vs_camera_aggregate=======
% \begin{figure}
% \centering
%     \includegraphics[width=7.5cm,height=6.0cm]{Images/allOnboardSensor_AOA_profile_3D_Traj.PNG}
%     \caption{\footnotesize{\emph{on-board sensor traj with 11\% elements that violate discretization threshold. groundtruth $\hat{\phi} = \ang{0}$, $\hat{\theta}=\ang{93.65}$. Estimated AOA $\phi = \ang{-0.5}$, $\theta=\ang{104.58}$}}}
%     \label{fig:Mocap_vs_camera_AOA}
% \end{figure}
% %========Mocap_Vs_camera_aggregate===========
% %====Impact of increasing inter-element spacing====
% \begin{figure*}
% 	    \centering
%         \includegraphics[width=15.0cm,height=8.0cm]{Images/Impact_of_increasing_inter-elememt-spacing.png}
%     	\caption{\footnotesize{\emph{ Shows the results of numerical analysis of Eqn~\ref{eqn:main_term_separate}, by comparing the ratio of main peak and anomalous peak, with inter-element spacing for an ideal 2D circular antenna array. Three sample simulated AoA profiles are shown where blue is the contribution of main peak (at $\phi$ = 180) and orange is the contribution of anomalous peaks in the profile. As evident from the profiles, with increased discretization, the ratio starts to drop; the anomalous peaks start to dominate leading to a noisy AoA profile.}}}
%     	\label{fig:Inter_element_spacing_numerical_results}
% \end{figure*}
% %====%====Impact of increasing inter-element spacing====
% \subsection{Comparison with Received Signal Strength Methods}
% \edit{To compare the AOA estimation accuracy of our system with compare it with existing methods. One of the commonly used approaches for estimating AOA is by using \emph{Received signal Strength Indicator} (RSSI). To improve the accuracy RSSI based approach, we use \emph{Effective Signal Strength Ratio} (ESNR) as it provides more granularity than RSSI and also maps directly to rate Mb/s thus acting as an indicator of signal quality~\citep{Halperin2010Predictable8P}. The quadrotor trajectories used to obtain wireless signal data have a helix geometry and 1.2 m long on average. Given the scenario we apply AoA finding, we need to treat existing trajectories as pre-collected offline samples instead of designing gradient descent controller to generate efficient samples. For every trial, we sample ESNR at each pose along the trajectory, choosing the AOA direction which has maximum increase in ESNR. We denote the normalized ESNR value at $i^{th}$ pose to be $ESNR_i$, $\eta$ as attenuation factors.} 
% % In order to obtain the AOA direction from sampled ESNR values, we formulate this problem as finding least square solution \textcolor{green}{$\tilde{\chi} = <x,y,z>$ - \textbf{duplicate notation}} utilizing the difference of $ESNR_{ij}$ at any pair of position $i$,$j$  in each trajectory as follow: 
% \begin{equation}
%     \label{eqn:esnr_least_square}
%     min\sum_{i\in [1,M], j\in [1,M], i\neq j}||ESNR_{ij} - \tilde{\chi} * (p_i-p_j)^T||_2
% \end{equation}
% %====Comparison with ESNR====
% \begin{figure}
% 		\centering
%         \includegraphics[width=8.5cm,height=6.5cm]{Images/ESNR_AOA_Accuracy_aerialRobot.PNG}
%     	\caption{\footnotesize{\emph{Aggregate AOA estimation Error over 101 hardware experiments comparing our method to ESNR based method for UAV. Our approach 3D trajectories obtained from motion capture for AOA estimation, while the ESNR based method does not rely on the trajectory itself, but requires sampling along different directions. Our approach shows better performance compared to ESNR based method, which suffers from lack of sampling.}}}
%     	\label{fig:Comparison_with_ESNR_drone}
% \end{figure}
% %====Comparison with ESNR====
% \noindent \edit{Fig.~\ref{fig:Comparison_with_ESNR_drone} shows the aggregate results that compare AOA accuracy using our approach and ESNR based approach. It is clear that our system performs much better compared to using ESNR for calculating AOA. The comparatively poor performance of ESNR based method can be attributed to the fact that it requires extensive sampling in different directions~\citep{Gil2015AdaptiveCI} to obtain the signal gradient fields. As this would involve modifying the trajectory of the robot to a large extent, it is not only time consuming but also constraints the type of motion the robot can perform. On the other hand, our method offers more flexibility by enabling AOA calculation over arbitrary trajectories. The Wi-Fi signal source robot is kept static during these experiments since it is required by ESNR based method, but is not a constraint for our system as shown in previous section.} 
%====Hardware experiment results- application ====
\begin{figure*}
	\centering
	\begin{minipage}{.495\linewidth}
		\centering
        \includegraphics[width=8.5cm,height=5.5cm]{Images/HW_implementation_img1.png}\\
        \footnotesize\emph{{(a) Initial setup}}
    	\vspace{7pt}
	\end{minipage}
% 	\hspace{10pt}
	\begin{minipage}{.495\linewidth}
		\centering
        \includegraphics[width=8.5cm,height=5.5cm]{Images/HW_implementation_img2.png}
        \footnotesize\emph{{(b) UAV starts navigating towards static ground robot}}
        \vspace{7pt}
	\end{minipage}
	\begin{minipage}{.495\linewidth}
		\centering
        \includegraphics[width=8.5cm,height=5.5cm]{Images/HW_implementation_img3.png}\\
        \footnotesize\emph{{(c) Ground robot starts to move and gets occluded}}
	\end{minipage}
% 	\hspace{2pt}
	\begin{minipage}{.495\linewidth}
		\centering
        \includegraphics[width=8.5cm,height=5.5cm]{Images/HW_implementation_img4.png}\\
        \footnotesize\emph{{(d) UAV achieves rendezvous with ground robot}}
	\end{minipage}
	\caption{\footnotesize\emph{{Shows different stages of dynamic rendezvous hardware experiment between signal transmitting ground robot and receiving UAV. Starting from top-left : a) The initial setup to test rendezvous of UAV with the ground robot in presence of occlusions. b) The UAV begins to navigate towards the stationary ground robot, leveraging relative AOA information obtained from continuously generating AOA profiles using our arbitrary 3D SAR system which leverages robot trajectory generated from its natural motion. c) The ground robot starts to move and gets occluded (UAV loses visual of the ground robot as seen in the fisheye view image). d) The UAV continues its navigation towards the ground robot despite of occlusion until it is within 2 meters proximity, at which point rendezvous is declared successful.}}}
    \label{fig:HW_application}
\end{figure*}
%====Hardware experiment results - application====
\section{Application Study}
\subsection*{Dynamic rendezvous between ground/air robots} \label{sec:hardware_application}
In this section, we demonstrate the performance of our system for a complete experiment of multi-robot rendezvous task between a UAV (signal receiving) and a ground robot (signal transmitting), so as to evaluate the utility of our system for a multi-robot coordination application that involves a heterogeneous team of robots. Our evaluation is based on the following three criteria:
\begin{itemize}
    \item \emph{System performance in presence of occlusions}: We verify that the UAV can navigate towards the ground robot using relative $AOA_{max}$ by continuously generating AOA profiles $F_{ij}(\phi,\theta)$ in realtime, even when the ground robot is occluded. 
    \item \emph{Performance of our system in the presence of moving ends}: We verify that the UAV continues it's navigation accurately even when the ground robot starts to move.
    \item \emph{Impact of trajectory geometry}: Following the development in Sec.~\ref{sec:cr-bound} we calculate the informativeness of trajectory geometry for each iteration of 3D SAR as the UAV navigates towards the ground robot.
\end{itemize}
% To showcase the utility of our system for different multi-robot applications, we conducted a proof of concept experiment where a UAV rendezvous with a moving ground robot in the presence of occlusion. Motion capture system is used to obtain the trajectory estimates required for AOA estimation instead of tacking camera to a) get benchmark performance for our application and b) address the lack of features that encompasses the entirety of the testbed which would adversely impact the performance of tracking camera.

\begin{figure*}%=======HW application stats============
    \centering
    \includegraphics[width=17.2cm,height=9.5cm]{Images/hw_exp_end_to_end_proof_of_concept_AOA_error_stats.png}
	\caption{\footnotesize{\emph{Plot showing $AOA_{Error}$ (Eqn.\ref{eqn:AOA_euclidean_error}) for signal receiving UAV during the dynamic rendezvous hardware experiment. Our approach takes into account the motion of transmitting robot (start indicated by vertical dotted line) while the UAV continues to navigate towards it. During each SAR iteration, the UAV travels a distance of 1.2 meter on average. AOA profiles and the UAV trajectory are shown for iteration 7 (point A) and iteration 9 (point B). High error at point B is due to low informativeness of the corresponding trajectory (show on the right) and an ambiguous $F_{ij}(\phi,\theta)$ (shown at the top). Similar behavior is observed for iteration 4. Conversely, the UAV trajectory at point A is highly informative and has almost no ambiguity leading to low $AOA_{Error}$. High AOA error for the first two iterations is due sudden jerk and high vibrations of the UAV chassis during take-off.}}}
	\label{fig:HW_application_stats}
\end{figure*}%=======HW application stats============
\begin{figure}%=======HW application stats 2 ============
        \includegraphics[width=8.5cm,height=5.0cm]{Images/hw_exp_end_to_end_proof_of_concept_AOA_error_stats_CRB_ERROR_v3.png}
	    \caption{\footnotesize{\emph{Shows that CRB can be used to presage AOA accuracy that would result from low informative trajectories. The results are for trajectories obtained during the dynamic rendezvous hardware experiment. The high CRB values at timesteps 4 and 9 indicate lower trajectory informativeness and higher ambiguity in $F_{ij}(\phi,\theta)$ (see Fig.~\ref{fig:HW_application_stats}). Correspondingly we see high $AOA_{Error}$ at those points. We note that despite the CRB being low for the first two iterations, the $AOA_{Error}$ is high, generally due sudden jerk and high vibrations of the UAV  chassis.}}}
    	\label{fig:HW_application_stats_crb_error}
\end{figure}%=======HW application stats 2 ============
\subsubsection*{\textbf{Experimental setup:}} We consider an environment of size 300 square meters with one aerial and one ground robot separated by distance 15m and visual occlusions due to a wall of cardboard boxes. We note that these occlusions block visual line-of-sight but are penetrable by WiFi signals. Motion capture is used to provide displacement information for the UAV (robot $i$). Information about the position of the ground robot (robot $j$) is not known to robot $i$ who solely uses obtained AOA information from its measured $F_{ij}(\phi,\theta)$ to track robot $j$. True AOA is obtained between robot $i$ and $j$ using their respective positions from motion capture system.

At the start of the experiment, the robots are separated by a distance of 15m (Fig.~\ref{fig:HW_application} (a)). The UAV, after take-off, starts to successfully navigate towards the ground robot, that is initially static, using relative $AOA_{max}$ obtained from wireless signal information and a simple waypoint motion controller (Fig.~\ref{fig:HW_application} (b)). The ground robot then starts to move and gets visually occluded by obstacles (Fig.~\ref{fig:HW_application} (c)), but the UAV continues to successfully navigate towards it. We consider the rendezvous successful when the UAV is within a 2m radius of the ground robot (Fig.~\ref{fig:HW_application} (d)). 

We note that as stated in Sec. \ref{sec:Problem Formulation}, the relative $AOA_{max}$ to the robot $j$ is calculated with respect to the initial position $p_i(t_k)$ of the robot $i$. Thus if the true AOA with respect to this initial position undergoes a substantial change over the data collection period, as could happen when agents are at short distances to one another or when robots are moving very fast relative to each other, then the $AOA_{max}$ will be outdated. For our experiments UAV and ground robot are traveling at 0.5 m/s and 0.1 m/s respectively and once they are within 2 meters of each other we stop tracking using $F_{ij}(\phi,\theta)$ (at this point we assume that an on-board camera could be used to maintain tracking).

\subsubsection*{\textbf{Evaluation:}} For evaluation of our system performance, we use $AOA_{Error}$ (Eqn. \ref{eqn:AOA_euclidean_error}) to measure the accuracy of our $AOA_{max}$ estimation against groundtruth (from motion capture). Our evaluation focuses on the following: 1) evaluating $AOA_{Error}$ over time, 2) evaluating $AOA_{Error}$ for the moving ends case where both the transmitting and receiving robots are moving, and 3) experimental characterization of the robot trajectory's \emph{informativeness} versus $AOA_{Error}$.

We collect data over UAV trajectories which are 1.2 m long on average to measure a complete $F_{ij}(\phi,\theta)$. We refer to this as a \emph{SAR iteration}. During a SAR iteration, the UAV uses its relative trajectory to generate $F_{ij}(\phi,\theta)$ and updates its waypoint to navigate towards the ground robot using estimated $AOA_{max}$ from $F_{ij}(\phi,\theta)$. Fig.~\ref{fig:HW_application_stats} shows the resulting accuracy of the $AOA_{max}$ estimation for each iteration. When the UAV initially takes-off, we observe high $AOA_{Error}$ (generally due sudden jerk and high vibrations of the chassis) before it stabilizes itself. Over the course of the experiment, the mean $AOA_{Error}$ between robots is 10.17 degrees with the exception of two outlier points at iteration 4 and 9. Note that $AOA_{Error}$ is not affected by the motion of the ground robot which begins at iteration 7. A closer look at iteration 9 and 4 reveals that the $F_{ij}(\phi,\theta)$ exhibits ambiguity peaks (ambiguous AOA directions) owing to sub-trajectories of low informativeness at these iterations (see Fig.~\ref{fig:HW_application_stats} top (b)). Intuitively, this occurs when the trajectory of the UAV resembles a 2D trajectory with little displacement along the z-axis and is predicted by a high CRB (low informativeness) value at these points in the experiment (see Fig.~\ref{fig:HW_application_stats_crb_error}). In contrast, all other iterations where the sub-trajectories of the UAV display high \emph{informativeness} as characterized by the CRB, result in more accurate, less ambiguous, AOA peaks as shown in Fig.~\ref{fig:HW_application_stats} top (a). 

\smallskip
\noindent We make the following important observations:
\begin{itemize}
    \item \emph{Accurate $AOA_{max}$ estimation with moving ends:} Despite the presence of a moving transmitting robot, our 3D SAR system enables the signal receiving UAV (robot $i$) to successfully achieve rendezvous by using relative trajectories that have high informativeness.
    \item \emph{Tracking through visual occlusions:} Our system enables the UAV to sense the ground robot's spatial direction despite the presence of visual occlusions.
    \item \emph{Informativeness as a predictor of AOA accuracy:} Iterations 4 and 9, which have high error in $AOA_{max}$ (Eqn.~\ref{eqn:AOA_euclidean_error}), have corresponding high CRB values indicating that these trajectories have low informativeness (Fig.~\ref{fig:HW_application_stats_crb_error}). By contrast, low CRB values correctly predict low $AOA_{Error}$.
\end{itemize}
\noindent Thus our experimental results support our theoretical developments with regards to addressing the moving ends problem, and characterizing the accuracy of measured $AOA_{max}$ as a function of the \emph{informativeness} of a robot's trajectory which is computable using Eqn.~\eqref{eq:CRB_helix_closed_form}.  Fig.~\ref{fig:HW_application_stats_crb_error} demonstrates the Cramer-Rao Bound (CRB) for each sub-trajectory of the UAV for each SAR iteration during the experiment. The CRB here is obtained via post-processing for the purposes of analysis.  We evaluate the CRB here using the true source direction.  Future implementations could consider online CRB computation using a \emph{worst-case} source direction which could then be used to \emph{optimize} robot trajectories for improved $AOA_{max}$ estimation.  We do not consider trajectory optimization here and rather leave this as an interesting direction of future work.

This proof-of-concept application study demonstrates the applicability of our developed framework to multi-robot tasks (e.g coverage or exploration) that require robots to maintain continuous mobility in an environment with obstacles and visual occlusions. Moreover, use of 3D robot trajectories during the task improves the information quality obtainable by our system. 

%\subsection{Feasibility of direction finding with Received Signal Strength} \label{sec:comparions_with_RSS}
%Here, we highlight some of the key observations from the experiment in Sec. \ref{sec:hardware_application} to show the challenges in using Received Signal Strength (RSS) for multi-robot applications, especially in indoor settings. As RSS information is coarse, it is not suitable for applications that require obtaining AOA information with small displacements. SAR-based methods in contrast, enable a signal receiving robot to find the direction of a transmitting robot in it's neighbourhood, with displacements as small as $2\lambda$ by measuring the change in phase of the signal. We note the following two observations pertaining to RSS during the dynamic rendezvous experiment:
%\begin{enumerate}
%    \item \emph{Variation in RSS for a given 3D trajectory of signal receiving robot:} As seen in Fig. \ref{fig:Comparison_with_RSS_rendezvous_application} (a), the measured RSS along the receiving robots arbitrary 3D trajectory does not allow for accurately distinguishing the direct signal path to the transmitting robot. As shown, the change in RSS level is within noise for robot displacements on the order of 1m.  
%    \item \emph{RSS value at the beginning and end of application experiment:} The robots are separated by a distance of 15m and 3m respectively, at the beginning and towards the end of the rendezvous experiment. RSS does indeed reflect improved signal strength over large differences in proximity (Fig. \ref{fig:Comparison_with_RSS_rendezvous_application} (a) and (b)), however observing such a clear trend requires large robot displacements and thus cannot be used effectively over smaller distances. 
%\end{enumerate}
%\noindent These observations match the analysis from theoretical models of RSS that conclude the same; i.e it is challenging to distinguish between positions that are within close proximity of each other in indoor environments \citep{Yang2013FromRT}. Thus an RSS based method would involve modifying the trajectory of the receiving robot to a greater extent so as to sample along different directions and find the one which leads to significant change as shown by \citep{Gil2015AdaptiveCI}. On the other hand, our method offers more flexibility by enabling AOA calculation over small arbitrary trajectories which are naturally generated by robots as they move. Another distinction between our approach and RSS based methods is the resolution of AOA information; our method gives spatial directions along azimuth and elevation separately while with RSS only a general direction of strongest signal might be obtained.
